A Differential Measurement of Circumstellar Extinction for AA Tau's 2011 Dimming Event

AA Tau is a classical T Tauri star with a highly inclined, warped circumstellar disk. For decades, AA Tau exhibited photometric and spectroscopic variability that were successfully modelled as occultations of the primary star by circumstellar material. In 2011, AA Tau entered an extended faint state, presumably due to enhanced levels of circumstellar dust. We use two sets of contemporaneous optical-NIR spectra of AA Tau, obtained in December of 2008 and 2014, to directly measure the wavelength-dependent extinction associated with the dust enhancement driving AA Tau's 2011 optical fade. Taken alone, AA Tau's apparent optical-NIR increased extinction curve cannot be fit well with standard extinction laws. At optical wavelengths, AA Tau's dimming event is consistent with predictions of common extinction models for an increase of $A_V=2$, but no such model reproduces AA Tau's color-color excess at NIR wavelengths. We show that veiling emission accounts for the apparent anomalous NIR extinction: after including this veiling flux, AA Tau's dimming event is consistent with a standard $A_V=2$ extinction law across the full optical-NIR range. We also report an increase in AA Tau's mid-IR flux since its 2011 fade, and suggest that an increase in the height of AA Tau's inner disk is the most likely explanation for both the IR brightening and the additional extinction along the line of sight. In addition to informing our understanding of AA Tau, this analysis demonstrates that caution should be exercised when inferring extinction (and stellar parameters) from the NIR color-color excess of young stars with measurable NIR veiling fluxes.

==> FormattedespadonsTable.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{ccccccccccccccccccccccc}
\tablewidth{0pt}
\tabletypesize{\tiny}
\tablecaption{Optical Veiling Measurements\label{tab:Opt_Veil}}
\tablehead{
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{5270} &
  \colhead{5270} &
  \colhead{5660} &
  \colhead{5660} &
  \colhead{Ca 6122} &
  \colhead{Ca 6122} &
  \colhead{6500} &
  \colhead{6500} &
  \colhead{Li 6708} &
  \colhead{Li 6708} &
  \colhead{K 7016} & 
  \colhead{K 7016} &
  \colhead{K 7326} &
  \colhead{K 7326} &
  \colhead{K 7700} &
  \colhead{K 7700} &
  \colhead{Fe 8689} &
  \colhead{Fe 8689} &
  \colhead{Mg 8807} &
  \colhead{Mg 8807} \\
  \colhead{MJD} &
  \colhead{$i$ flux} &
  \colhead{$i$ Mag} &
  \colhead{Flux} &
  \colhead{EqW} &
  \colhead{Flux} &
  \colhead{EqW} &
  \colhead{Flux} &
  \colhead{EqW} &
  \colhead{Flux} &
  \colhead{EqW} &
  \colhead{Flux} &
  \colhead{EqW} &
  \colhead{Flux} & 
  \colhead{EqW} &
  \colhead{Flux} &
  \colhead{EqW} &
  \colhead{Flux} &
  \colhead{EqW} &
  \colhead{Flux} &
  \colhead{EqW} &
  \colhead{Flux} &
  \colhead{EqW} }

\startdata
54806.438 & 4.90 & -1.73 & 1.096E-02 & 4.636E-01 & 2.551E-03 & 9.462E-02 & 2.627E-03 & 8.833E-02 & 4.475E-03 & 1.397E-01 & 1.731E-03 & 5.754E-02 & 9.092E-04 & 2.553E-02 & 1.153E-03 & 3.076E-02 & 2.240E-03 & 5.565E-02 & 2.376E-03 & 4.777E-02 & 2.506E-03 & 4.688E-02 \\
54806.453 & 5.18 & -1.79 & 1.173E-02 & 4.650E-01 & 2.774E-03 & 9.634E-02 & 2.785E-03 & 8.806E-02 & 4.768E-03 & 1.402E-01 & 1.850E-03 & 5.758E-02 & 9.542E-04 & 2.532E-02 & 1.223E-03 & 3.079E-02 & 2.399E-03 & 5.618E-02 & 2.587E-03 & 4.906E-02 & 2.709E-03 & 4.774E-02 \\
54806.465 & 5.08 & -1.76 & 1.159E-02 & 4.697E-01 & 2.642E-03 & 9.409E-02 & 2.714E-03 & 8.797E-02 & 4.570E-03 & 1.382E-01 & 1.820E-03 & 5.850E-02 & 9.192E-04 & 2.498E-02 & 1.204E-03 & 3.100E-02 & 2.370E-03 & 5.633E-02 & 2.467E-03 & 4.791E-02 & 2.672E-03 & 4.793E-02 \\
54806.480 & 5.03 & -1.75 & 1.173E-02 & 4.755E-01 & 2.531E-03 & 9.133E-02 & 2.682E-03 & 8.719E-02 & 4.635E-03 & 1.405E-01 & 1.790E-03 & 5.789E-02 & 9.432E-04 & 2.567E-02 & 1.189E-03 & 3.083E-02 & 2.284E-03 & 5.537E-02 & 2.504E-03 & 4.885E-02 & 2.584E-03 & 4.713E-02 \\
54807.387 & 5.80 & -1.91 & 1.355E-02 & 4.630E-01 & 3.052E-03 & 9.209E-02 & 3.236E-03 & 8.840E-02 & 5.471E-03 & 1.404E-01 & 2.094E-03 & 5.715E-02 & 1.156E-03 & 2.676E-02 & 1.397E-03 & 3.115E-02 & 2.723E-03 & 5.603E-02 & 2.915E-03 & 4.937E-02 & 3.035E-03 & 4.820E-02 \\
54807.402 & 5.82 & -1.91 & 1.387E-02 & 4.721E-01 & 3.255E-03 & 9.739E-02 & 3.317E-03 & 8.988E-02 & 5.545E-03 & 1.417E-01 & 2.109E-03 & 5.746E-02 & 1.143E-03 & 2.657E-02 & 1.416E-03 & 3.137E-02 & 2.698E-03 & 5.552E-02 & 2.877E-03 & 4.855E-02 & 3.120E-03 & 4.906E-02 \\
54807.418 & 5.89 & -1.93 & 1.388E-02 & 4.647E-01 & 3.034E-03 & 8.984E-02 & 3.289E-03 & 8.852E-02 & 5.557E-03 & 1.404E-01 & 2.128E-03 & 5.716E-02 & 1.144E-03 & 2.631E-02 & 1.411E-03 & 3.103E-02 & 2.671E-03 & 5.435E-02 & 2.922E-03 & 4.892E-02 & 3.171E-03 & 4.937E-02 \\
54807.430 & 5.89 & -1.93 & 1.407E-02 & 4.701E-01 & 3.236E-03 & 9.536E-02 & 3.270E-03 & 8.778E-02 & 5.514E-03 & 1.389E-01 & 2.129E-03 & 5.708E-02 & 1.215E-03 & 2.768E-02 & 1.394E-03 & 3.063E-02 & 2.745E-03 & 5.567E-02 & 2.934E-03 & 4.893E-02 & 3.090E-03 & 4.809E-02 \\
54808.406 & 4.09 & -1.53 & 8.372E-03 & 4.620E-01 & 1.958E-03 & 9.359E-02 & 2.076E-03 & 8.798E-02 & 3.628E-03 & 1.407E-01 & 1.394E-03 & 5.745E-02 & 7.306E-04 & 2.526E-02 & 9.363E-04 & 3.049E-02 & 1.897E-03 & 5.667E-02 & 1.932E-03 & 4.595E-02 & 2.163E-03 & 4.725E-02 \\
54808.422 & 4.03 & -1.51 & 8.422E-03 & 4.675E-01 & 1.774E-03 & 8.707E-02 & 2.044E-03 & 8.821E-02 & 3.562E-03 & 1.406E-01 & 1.319E-03 & 5.566E-02 & 7.252E-04 & 2.533E-02 & 9.290E-04 & 3.075E-02 & 1.869E-03 & 5.679E-02 & 1.936E-03 & 4.645E-02 & 2.017E-03 & 4.512E-02 \\
54808.438 & 3.68 & -1.42 & 7.376E-03 & 4.610E-01 & 1.751E-03 & 9.398E-02 & 1.864E-03 & 8.886E-02 & 3.236E-03 & 1.417E-01 & 1.212E-03 & 5.617E-02 & 6.348E-04 & 2.461E-02 & 8.387E-04 & 3.031E-02 & 1.697E-03 & 5.674E-02 & 1.845E-03 & 4.782E-02 & 1.972E-03 & 4.758E-02 \\
54808.449 & 3.63 & -1.40 & 7.245E-03 & 4.616E-01 & 1.633E-03 & 8.963E-02 & 1.786E-03 & 8.699E-02 & 3.078E-03 & 1.374E-01 & 1.214E-03 & 5.692E-02 & 6.213E-04 & 2.457E-02 & 8.182E-04 & 3.019E-02 & 1.644E-03 & 5.578E-02 & 1.781E-03 & 4.716E-02 & 1.877E-03 & 4.613E-02 \\
54809.406 & 2.19 & -0.85 & 4.775E-03 & 4.571E-01 & 1.171E-03 & 9.683E-02 & 1.170E-03 & 8.825E-02 & 1.874E-03 & 1.331E-01 & 7.626E-04 & 5.682E-02 & 4.294E-04 & 2.705E-02 & 5.161E-04 & 3.111E-02 & 9.838E-04 & 5.490E-02 & 1.079E-03 & 4.801E-02 & 1.159E-03 & 4.794E-02 \\
54809.422 & 3.65 & -1.41 & 7.967E-03 & 4.538E-01 & 1.814E-03 & 9.055E-02 & 1.959E-03 & 8.888E-02 & 3.296E-03 & 1.393E-01 & 1.273E-03 & 5.715E-02 & 6.519E-04 & 2.489E-02 & 8.418E-04 & 3.050E-02 & 1.675E-03 & 5.603E-02 & 1.829E-03 & 4.828E-02 & 1.929E-03 & 4.766E-02 \\
54809.438 & 2.47 & -0.98 & 5.617E-03 & 4.619E-01 & 1.238E-03 & 9.060E-02 & 1.317E-03 & 8.818E-02 & 2.267E-03 & 1.407E-01 & 8.576E-04 & 5.668E-02 & 4.611E-04 & 2.569E-02 & 5.350E-04 & 2.864E-02 & 1.112E-03 & 5.502E-02 & 1.177E-03 & 4.645E-02 & 1.310E-03 & 4.743E-02 \\
54809.453 & 2.38 & -0.94 & 5.417E-03 & 4.587E-01 & 1.095E-03 & 8.338E-02 & 1.285E-03 & 8.707E-02 & 2.153E-03 & 1.373E-01 & 8.341E-04 & 5.631E-02 & 4.460E-04 & 2.572E-02 & 5.665E-04 & 3.120E-02 & 1.069E-03 & 5.459E-02 & 1.159E-03 & 4.736E-02 & 1.274E-03 & 4.815E-02 \\
54810.395 & 1.57 & -0.49 & 2.868E-03 & 4.495E-01 & 6.020E-04 & 8.130E-02 & 7.352E-04 & 8.544E-02 & 1.232E-03 & 1.307E-01 & 5.022E-04 & 5.622E-02 & 2.285E-04 & 2.140E-02 & 3.534E-04 & 3.077E-02 & 7.185E-04 & 5.746E-02 & 6.965E-04 & 4.278E-02 & 7.841E-04 & 4.384E-02 \\
54810.410 & 1.48 & -0.42 & 2.629E-03 & 4.453E-01 & 5.340E-04 & 7.844E-02 & 7.016E-04 & 8.719E-02 & 1.185E-03 & 1.374E-01 & 4.659E-04 & 5.655E-02 & 2.250E-04 & 2.266E-02 & 3.248E-04 & 3.036E-02 & 6.485E-04 & 5.557E-02 & 7.154E-04 & 4.552E-02 & 7.482E-04 & 4.431E-02 \\
54810.426 & 1.21 & -0.21 & 2.240E-03 & 4.445E-01 & 6.083E-04 & 1.015E-01 & 5.688E-04 & 8.456E-02 & 1.027E-03 & 1.396E-01 & 4.178E-04 & 5.730E-02 & 1.994E-04 & 2.390E-02 & 2.741E-04 & 3.079E-02 & 5.176E-04 & 5.397E-02 & 5.727E-04 & 4.527E-02 & 6.022E-04 & 4.383E-02 \\
54810.438 & 1.78 & -0.63 & 3.470E-03 & 4.449E-01 & 7.271E-04 & 8.242E-02 & 8.872E-04 & 8.751E-02 & 1.494E-03 & 1.358E-01 & 5.593E-04 & 5.422E-02 & 3.119E-04 & 2.489E-02 & 3.742E-04 & 2.850E-02 & 7.728E-04 & 5.401E-02 & 7.842E-04 & 4.253E-02 & 8.379E-04 & 4.157E-02 \\
54815.391 & 4.75 & -1.69 & 1.038E-02 & 4.527E-01 & 2.477E-03 & 9.406E-02 & 2.483E-03 & 8.594E-02 & 4.289E-03 & 1.385E-01 & 1.632E-03 & 5.620E-02 & 8.325E-04 & 2.431E-02 & 1.102E-03 & 3.043E-02 & 2.208E-03 & 5.622E-02 & 2.365E-03 & 4.862E-02 & 2.481E-03 & 4.769E-02 \\
54815.406 & 5.45 & -1.84 & 1.209E-02 & 4.553E-01 & 2.728E-03 & 9.040E-02 & 2.903E-03 & 8.710E-02 & 4.900E-03 & 1.376E-01 & 1.861E-03 & 5.563E-02 & 9.705E-04 & 2.471E-02 & 1.260E-03 & 3.032E-02 & 2.499E-03 & 5.549E-02 & 2.643E-03 & 4.764E-02 & 2.804E-03 & 4.712E-02 \\
54815.422 & 5.59 & -1.87 & 1.266E-02 & 4.600E-01 & 2.819E-03 & 9.072E-02 & 2.948E-03 & 8.624E-02 & 5.074E-03 & 1.383E-01 & 1.948E-03 & 5.649E-02 & 1.010E-03 & 2.495E-02 & 1.295E-03 & 3.038E-02 & 2.556E-03 & 5.542E-02 & 2.701E-03 & 4.761E-02 & 2.896E-03 & 4.764E-02 \\
54815.438 & 5.28 & -1.81 & 1.187E-02 & 4.587E-01 & 2.569E-03 & 8.916E-02 & 2.770E-03 & 8.639E-02 & 4.720E-03 & 1.375E-01 & 1.833E-03 & 5.662E-02 & 9.569E-04 & 2.507E-02 & 1.237E-03 & 3.068E-02 & 2.379E-03 & 5.489E-02 & 2.573E-03 & 4.773E-02 & 2.737E-03 & 4.738E-02 \\
54816.375 & 2.53 & -1.01 & 5.492E-03 & 4.410E-01 & 1.157E-03 & 8.285E-02 & 1.320E-03 & 8.530E-02 & 2.175E-03 & 1.318E-01 & 8.580E-04 & 5.428E-02 & 4.504E-04 & 2.474E-02 & 5.683E-04 & 2.967E-02 & 1.123E-03 & 5.350E-02 & 1.154E-03 & 4.492E-02 & 1.261E-03 & 4.528E-02 \\
54816.391 & 1.28 & -0.27 & 2.740E-03 & 4.437E-01 & 6.583E-04 & 9.192E-02 & 6.462E-04 & 8.256E-02 & 1.087E-03 & 1.305E-01 & 4.282E-04 & 5.380E-02 & 2.214E-04 & 2.404E-02 & 2.796E-04 & 2.898E-02 & 5.563E-04 & 5.237E-02 & 6.265E-04 & 4.717E-02 & 6.243E-04 & 4.448E-02 \\
54816.406 & 1.19 & -0.19 & 2.589E-03 & 4.482E-01 & 5.673E-04 & 8.809E-02 & 5.986E-04 & 8.318E-02 & 1.086E-03 & 1.403E-01 & 4.124E-04 & 5.440E-02 & 1.960E-04 & 2.315E-02 & 2.658E-04 & 2.988E-02 & 5.360E-04 & 5.414E-02 & 5.539E-04 & 4.525E-02 & 5.799E-04 & 4.403E-02 \\
54816.418 & 0.29 & 1.33 & 6.684E-04 & 4.330E-01 & 1.970E-04 & 1.095E-01 & 1.346E-04 & 7.232E-02 & 2.636E-04 & 1.331E-01 & 9.023E-05 & 4.541E-02 & 4.848E-05 & 2.285E-02 & 6.347E-05 & 2.806E-02 & 1.130E-04 & 4.664E-02 & 1.350E-04 & 4.561E-02 & 1.719E-04 & 5.264E-02 \\
54817.367 & 3.28 & -1.29 & 6.830E-03 & 3.949E-01 & 1.528E-03 & 7.965E-02 & 1.692E-03 & 8.057E-02 & 2.679E-03 & 1.210E-01 & 1.091E-03 & 5.201E-02 & 6.157E-04 & 2.547E-02 & 7.752E-04 & 3.036E-02 & 1.487E-03 & 5.417E-02 & 1.474E-03 & 4.422E-02 & 1.501E-03 & 4.190E-02 \\
54817.383 & 1.44 & -0.40 & 3.105E-03 & 4.090E-01 & 7.138E-04 & 8.458E-02 & 7.187E-04 & 7.925E-02 & 1.192E-03 & 1.236E-01 & 4.804E-04 & 5.229E-02 & 2.780E-04 & 2.641E-02 & 3.244E-04 & 2.922E-02 & 6.449E-04 & 5.362E-02 & 6.669E-04 & 4.522E-02 & 7.126E-04 & 4.536E-02 \\
54817.398 & 5.11 & -1.77 & 1.075E-02 & 3.978E-01 & 2.379E-03 & 8.001E-02 & 2.573E-03 & 7.933E-02 & 4.378E-03 & 1.268E-01 & 1.618E-03 & 4.956E-02 & 9.499E-04 & 2.541E-02 & 1.209E-03 & 3.057E-02 & 2.263E-03 & 5.323E-02 & 2.230E-03 & 4.299E-02 & 2.415E-03 & 4.316E-02 \\
54817.414 & 5.43 & -1.84 & 1.127E-02 & 3.943E-01 & 2.600E-03 & 8.203E-02 & 2.744E-03 & 7.959E-02 & 4.731E-03 & 1.285E-01 & 1.803E-03 & 5.217E-02 & 1.008E-03 & 2.531E-02 & 1.307E-03 & 3.104E-02 & 2.367E-03 & 5.234E-02 & 2.389E-03 & 4.298E-02 & 2.547E-03 & 4.273E-02 \\
54818.363 & 3.95 & -1.49 & 7.809E-03 & 4.199E-01 & 1.708E-03 & 8.130E-02 & 1.968E-03 & 8.411E-02 & 3.282E-03 & 1.297E-01 & 1.253E-03 & 5.290E-02 & 7.715E-04 & 2.732E-02 & 9.893E-04 & 3.290E-02 & 1.700E-03 & 5.262E-02 & 1.719E-03 & 4.201E-02 & 1.950E-03 & 4.389E-02 \\
54818.379 & 4.10 & -1.53 & 8.174E-03 & 4.203E-01 & 1.774E-03 & 8.082E-02 & 2.054E-03 & 8.362E-02 & 3.189E-03 & 1.215E-01 & 1.326E-03 & 5.375E-02 & 7.604E-04 & 2.622E-02 & 1.004E-03 & 3.224E-02 & 1.792E-03 & 5.327E-02 & 1.811E-03 & 4.265E-02 & 1.999E-03 & 4.349E-02 \\
54818.395 & 4.07 & -1.52 & 7.941E-03 & 4.123E-01 & 1.647E-03 & 7.663E-02 & 2.014E-03 & 8.284E-02 & 3.380E-03 & 1.293E-01 & 1.297E-03 & 5.282E-02 & 7.753E-04 & 2.685E-02 & 9.663E-04 & 3.149E-02 & 1.778E-03 & 5.345E-02 & 1.834E-03 & 4.342E-02 & 2.070E-03 & 4.538E-02 \\
54818.410 & 3.93 & -1.49 & 7.887E-03 & 4.223E-01 & 1.769E-03 & 8.353E-02 & 1.935E-03 & 8.299E-02 & 3.234E-03 & 1.291E-01 & 1.280E-03 & 5.384E-02 & 7.288E-04 & 2.621E-02 & 9.220E-04 & 3.104E-02 & 1.739E-03 & 5.375E-02 & 1.756E-03 & 4.288E-02 & 2.006E-03 & 4.522E-02 \\
54819.363 & 2.31 & -0.91 & 4.011E-03 & 4.178E-01 & 9.156E-04 & 8.230E-02 & 1.045E-03 & 8.297E-02 & 1.760E-03 & 1.275E-01 & 6.756E-04 & 5.189E-02 & 3.940E-04 & 2.494E-02 & 5.150E-04 & 3.035E-02 & 9.894E-04 & 5.342E-02 & 1.072E-03 & 4.353E-02 & 1.072E-03 & 4.043E-02 \\
54819.379 & 1.96 & -0.73 & 3.396E-03 & 4.253E-01 & 7.499E-04 & 8.213E-02 & 8.621E-04 & 8.265E-02 & 1.451E-03 & 1.261E-01 & 5.759E-04 & 5.292E-02 & 3.131E-04 & 2.374E-02 & 4.451E-04 & 3.127E-02 & 8.394E-04 & 5.383E-02 & 8.403E-04 & 4.070E-02 & 9.310E-04 & 4.100E-02 \\
54819.395 & 2.11 & -0.81 & 3.606E-03 & 4.102E-01 & 8.914E-04 & 8.715E-02 & 9.815E-04 & 8.472E-02 & 1.659E-03 & 1.312E-01 & 6.125E-04 & 5.134E-02 & 3.624E-04 & 2.502E-02 & 4.705E-04 & 3.012E-02 & 8.681E-04 & 5.166E-02 & 9.862E-04 & 4.381E-02 & 1.016E-03 & 4.151E-02 \\
54819.410 & 2.13 & -0.82 & 3.733E-03 & 4.236E-01 & 8.338E-04 & 8.274E-02 & 9.931E-04 & 8.558E-02 & 1.712E-03 & 1.350E-01 & 6.158E-04 & 5.132E-02 & 3.509E-04 & 2.423E-02 & 4.741E-04 & 3.045E-02 & 8.974E-04 & 5.270E-02 & 9.374E-04 & 4.138E-02 & 1.042E-03 & 4.195E-02 \\
54820.363 & 1.31 & -0.30 & 2.482E-03 & 4.562E-01 & 5.742E-04 & 9.071E-02 & 6.088E-04 & 8.488E-02 & 1.073E-03 & 1.356E-01 & 4.065E-04 & 5.479E-02 & 2.178E-04 & 2.388E-02 & 2.928E-04 & 3.018E-02 & 6.138E-04 & 5.862E-02 & 6.297E-04 & 4.639E-02 & 6.505E-04 & 4.405E-02 \\
54820.379 & 2.82 & -1.13 & 5.518E-03 & 4.432E-01 & 1.262E-03 & 8.869E-02 & 1.350E-03 & 8.503E-02 & 2.184E-03 & 1.268E-01 & 9.076E-04 & 5.604E-02 & 4.898E-04 & 2.469E-02 & 6.408E-04 & 3.048E-02 & 1.272E-03 & 5.660E-02 & 1.272E-03 & 4.327E-02 & 1.469E-03 & 4.585E-02 \\
54820.395 & 3.83 & -1.46 & 7.375E-03 & 4.356E-01 & 1.640E-03 & 8.546E-02 & 1.864E-03 & 8.546E-02 & 3.043E-03 & 1.298E-01 & 1.231E-03 & 5.597E-02 & 6.300E-04 & 2.347E-02 & 8.541E-04 & 2.994E-02 & 1.746E-03 & 5.706E-02 & 1.750E-03 & 4.426E-02 & 2.010E-03 & 4.632E-02 \\
54820.406 & 3.93 & -1.49 & 7.737E-03 & 4.398E-01 & 1.727E-03 & 8.724E-02 & 1.894E-03 & 8.544E-02 & 3.164E-03 & 1.309E-01 & 1.255E-03 & 5.563E-02 & 6.519E-04 & 2.362E-02 & 8.798E-04 & 3.020E-02 & 1.775E-03 & 5.658E-02 & 1.818E-03 & 4.459E-02 & 2.054E-03 & 4.592E-02 \\
54838.254 & 4.22 & -1.56 & 9.406E-03 & 4.736E-01 & 1.991E-03 & 8.952E-02 & 2.176E-03 & 8.782E-02 & 3.868E-03 & 1.433E-01 & 1.445E-03 & 5.718E-02 & 7.269E-04 & 2.402E-02 & 9.755E-04 & 3.060E-02 & 1.928E-03 & 5.672E-02 & 2.068E-03 & 4.757E-02 & 2.217E-03 & 4.732E-02 \\
54838.270 & 4.32 & -1.59 & 9.519E-03 & 4.689E-01 & 2.113E-03 & 9.145E-02 & 2.332E-03 & 9.059E-02 & 3.893E-03 & 1.403E-01 & 1.491E-03 & 5.747E-02 & 7.065E-04 & 2.299E-02 & 1.065E-03 & 3.230E-02 & 1.997E-03 & 5.697E-02 & 2.096E-03 & 4.727E-02 & 2.296E-03 & 4.763E-02 \\
54838.285 & 4.51 & -1.64 & 9.993E-03 & 4.682E-01 & 2.281E-03 & 9.362E-02 & 2.369E-03 & 8.840E-02 & 4.057E-03 & 1.396E-01 & 1.551E-03 & 5.735E-02 & 7.963E-04 & 2.454E-02 & 1.077E-03 & 3.130E-02 & 2.081E-03 & 5.709E-02 & 2.181E-03 & 4.731E-02 & 2.410E-03 & 4.791E-02 \\
54838.297 & 4.82 & -1.71 & 1.089E-02 & 4.694E-01 & 2.366E-03 & 9.072E-02 & 2.605E-03 & 8.947E-02 & 4.416E-03 & 1.413E-01 & 1.669E-03 & 5.740E-02 & 8.255E-04 & 2.382E-02 & 1.144E-03 & 3.116E-02 & 2.268E-03 & 5.808E-02 & 2.404E-03 & 4.868E-02 & 2.637E-03 & 4.940E-02 \\
54840.223 & 4.20 & -1.56 & 9.888E-03 & 4.620E-01 & 2.186E-03 & 9.187E-02 & 2.262E-03 & 8.607E-02 & 3.831E-03 & 1.361E-01 & 1.511E-03 & 5.660E-02 & 7.758E-04 & 2.488E-02 & 1.006E-03 & 3.081E-02 & 1.925E-03 & 5.455E-02 & 2.094E-03 & 4.873E-02 & 2.223E-03 & 4.877E-02 \\
54840.238 & 4.63 & -1.67 & 1.082E-02 & 4.584E-01 & 2.361E-03 & 8.918E-02 & 2.481E-03 & 8.533E-02 & 4.261E-03 & 1.364E-01 & 1.663E-03 & 5.639E-02 & 8.218E-04 & 2.396E-02 & 1.127E-03 & 3.127E-02 & 2.160E-03 & 5.544E-02 & 2.276E-03 & 4.862E-02 & 2.387E-03 & 4.759E-02 \\
54840.250 & 5.15 & -1.78 & 1.216E-02 & 4.571E-01 & 2.822E-03 & 9.412E-02 & 2.822E-03 & 8.643E-02 & 4.831E-03 & 1.381E-01 & 1.858E-03 & 5.630E-02 & 9.681E-04 & 2.517E-02 & 1.264E-03 & 3.133E-02 & 2.377E-03 & 5.497E-02 & 2.506E-03 & 4.828E-02 & 2.723E-03 & 4.899E-02 \\
54840.266 & 5.06 & -1.76 & 1.231E-02 & 4.631E-01 & 2.742E-03 & 9.316E-02 & 2.776E-03 & 8.623E-02 & 4.685E-03 & 1.361E-01 & 1.843E-03 & 5.673E-02 & 9.388E-04 & 2.486E-02 & 1.199E-03 & 3.034E-02 & 2.313E-03 & 5.456E-02 & 2.470E-03 & 4.833E-02 & 2.645E-03 & 4.839E-02 \\
54841.215 & 5.59 & -1.87 & 1.355E-02 & 4.644E-01 & 3.206E-03 & 9.701E-02 & 3.097E-03 & 8.683E-02 & 5.158E-03 & 1.349E-01 & 2.023E-03 & 5.636E-02 & 1.040E-03 & 2.486E-02 & 1.369E-03 & 3.152E-02 & 2.572E-03 & 5.490E-02 & 2.636E-03 & 4.663E-02 & 2.909E-03 & 4.777E-02 \\
54841.230 & 5.50 & -1.85 & 1.334E-02 & 4.644E-01 & 2.988E-03 & 9.276E-02 & 3.029E-03 & 8.595E-02 & 5.286E-03 & 1.398E-01 & 2.004E-03 & 5.651E-02 & 9.965E-04 & 2.438E-02 & 1.350E-03 & 3.156E-02 & 2.515E-03 & 5.463E-02 & 2.715E-03 & 4.844E-02 & 2.928E-03 & 4.861E-02 \\
54841.242 & 5.71 & -1.89 & 1.401E-02 & 4.650E-01 & 3.083E-03 & 9.169E-02 & 3.287E-03 & 8.907E-02 & 5.462E-03 & 1.391E-01 & 2.124E-03 & 5.747E-02 & 1.033E-03 & 2.431E-02 & 1.363E-03 & 3.066E-02 & 2.601E-03 & 5.457E-02 & 2.818E-03 & 4.847E-02 & 3.021E-03 & 4.837E-02 \\
54841.258 & 5.67 & -1.88 & 1.389E-02 & 4.646E-01 & 3.045E-03 & 9.132E-02 & 3.237E-03 & 8.859E-02 & 5.373E-03 & 1.379E-01 & 2.083E-03 & 5.678E-02 & 1.057E-03 & 2.508E-02 & 1.374E-03 & 3.116E-02 & 2.551E-03 & 5.406E-02 & 2.797E-03 & 4.842E-02 & 3.047E-03 & 4.913E-02 \\
54842.227 & 2.25 & -0.88 & 4.534E-03 & 4.637E-01 & 9.971E-04 & 8.937E-02 & 1.117E-03 & 8.812E-02 & 1.822E-03 & 1.327E-01 & 7.264E-04 & 5.591E-02 & 3.636E-04 & 2.328E-02 & 5.248E-04 & 3.130E-02 & 1.007E-03 & 5.564E-02 & 1.106E-03 & 4.679E-02 & 1.207E-03 & 4.702E-02 \\
54842.242 & 2.48 & -0.98 & 5.064E-03 & 4.648E-01 & 1.218E-03 & 9.732E-02 & 1.190E-03 & 8.452E-02 & 2.080E-03 & 1.365E-01 & 8.259E-04 & 5.713E-02 & 4.027E-04 & 2.334E-02 & 5.838E-04 & 3.152E-02 & 1.129E-03 & 5.634E-02 & 1.208E-03 & 4.681E-02 & 1.343E-03 & 4.764E-02 \\
54842.367 & 2.70 & -1.08 & 5.442E-03 & 4.592E-01 & 1.172E-03 & 8.730E-02 & 1.330E-03 & 8.730E-02 & 2.292E-03 & 1.382E-01 & 9.208E-04 & 5.861E-02 & 4.623E-04 & 2.432E-02 & 6.175E-04 & 3.070E-02 & 1.260E-03 & 5.771E-02 & 1.329E-03 & 4.688E-02 & 1.450E-03 & 4.703E-02 \\
54842.383 & 3.01 & -1.20 & 6.042E-03 & 4.551E-01 & 1.423E-03 & 9.341E-02 & 1.504E-03 & 8.864E-02 & 2.599E-03 & 1.408E-01 & 1.037E-03 & 5.908E-02 & 5.121E-04 & 2.440E-02 & 6.937E-04 & 3.109E-02 & 1.331E-03 & 5.501E-02 & 1.488E-03 & 4.694E-02 & 1.649E-03 & 4.789E-02 \\
54842.398 & 3.34 & -1.31 & 6.807E-03 & 4.626E-01 & 1.501E-03 & 8.926E-02 & 1.666E-03 & 8.755E-02 & 2.798E-03 & 1.364E-01 & 1.110E-03 & 5.735E-02 & 5.769E-04 & 2.443E-02 & 7.709E-04 & 3.091E-02 & 1.550E-03 & 5.691E-02 & 1.625E-03 & 4.667E-02 & 1.863E-03 & 4.883E-02 \\
54842.410 & 3.36 & -1.31 & 6.854E-03 & 4.644E-01 & 1.560E-03 & 9.299E-02 & 1.665E-03 & 8.772E-02 & 2.845E-03 & 1.385E-01 & 1.121E-03 & 5.734E-02 & 5.867E-04 & 2.482E-02 & 7.718E-04 & 3.081E-02 & 1.606E-03 & 5.880E-02 & 1.664E-03 & 4.753E-02 & 1.774E-03 & 4.648E-02 \\
54843.215 & 0.05 & 3.16 & 1.585E-04 & 5.742E-01 & 1.374E-05 & 4.822E-02 & 3.043E-05 & 1.015E-01 & 3.306E-05 & 9.166E-02 & 1.836E-05 & 4.697E-02 & 1.032E-05 & 2.458E-02 & 1.401E-05 & 3.467E-02 & 2.292E-05 & 5.404E-02 & 3.462E-05 & 5.454E-02 & 3.471E-05 & 5.286E-02 \\
54843.230 & 0.29 & 1.35 & 5.868E-04 & 4.692E-01 & 1.060E-04 & 8.011E-02 & 1.484E-04 & 9.211E-02 & 1.714E-04 & 1.006E-01 & 8.849E-05 & 5.219E-02 & 5.287E-05 & 2.527E-02 & 5.708E-05 & 2.650E-02 & 1.285E-04 & 5.651E-02 & 1.224E-04 & 4.236E-02 & 1.730E-04 & 5.286E-02 \\
54843.246 & 1.10 & -0.10 & 2.158E-03 & 4.514E-01 & 4.454E-04 & 8.254E-02 & 5.376E-04 & 8.884E-02 & 8.848E-04 & 1.352E-01 & 3.764E-04 & 6.034E-02 & 1.885E-04 & 2.446E-02 & 2.386E-04 & 2.957E-02 & 5.000E-04 & 5.660E-02 & 5.565E-04 & 4.826E-02 & 5.407E-04 & 4.382E-02 \\
54843.262 & 1.18 & -0.18 & 2.331E-03 & 4.452E-01 & 4.972E-04 & 8.490E-02 & 5.833E-04 & 8.664E-02 & 1.007E-03 & 1.379E-01 & 3.816E-04 & 5.553E-02 & 1.985E-04 & 2.356E-02 & 2.529E-04 & 2.858E-02 & 5.463E-04 & 5.720E-02 & 6.023E-04 & 4.875E-02 & 6.011E-04 & 4.494E-02 \\
54843.277 & 1.64 & -0.54 & 3.260E-03 & 4.566E-01 & 7.260E-04 & 9.029E-02 & 8.272E-04 & 9.045E-02 & 1.348E-03 & 1.368E-01 & 5.331E-04 & 5.725E-02 & 2.567E-04 & 2.258E-02 & 3.694E-04 & 3.029E-02 & 7.481E-04 & 5.740E-02 & 7.973E-04 & 4.681E-02 & 8.432E-04 & 4.516E-02 \\
54843.289 & 2.17 & -0.84 & 4.209E-03 & 4.519E-01 & 1.014E-03 & 9.500E-02 & 1.089E-03 & 9.078E-02 & 1.762E-03 & 1.358E-01 & 7.270E-04 & 5.916E-02 & 3.403E-04 & 2.257E-02 & 4.834E-04 & 3.003E-02 & 9.611E-04 & 5.610E-02 & 1.066E-03 & 4.708E-02 & 1.212E-03 & 4.842E-02 \\
54843.305 & 3.27 & -1.29 & 6.445E-03 & 4.568E-01 & 1.471E-03 & 9.107E-02 & 1.615E-03 & 8.856E-02 & 2.652E-03 & 1.345E-01 & 1.094E-03 & 5.913E-02 & 5.470E-04 & 2.396E-02 & 7.608E-04 & 3.129E-02 & 1.553E-03 & 5.934E-02 & 1.596E-03 & 4.666E-02 & 1.759E-03 & 4.673E-02 \\
54844.199 & 3.02 & -1.20 & 6.073E-03 & 4.788E-01 & 1.269E-03 & 8.828E-02 & 1.496E-03 & 9.003E-02 & 2.401E-03 & 1.327E-01 & 9.725E-04 & 5.748E-02 & 5.237E-04 & 2.474E-02 & 7.803E-04 & 3.428E-02 & 1.398E-03 & 5.738E-02 & 1.537E-03 & 4.761E-02 & 1.643E-03 & 4.672E-02 \\
54844.211 & 2.67 & -1.06 & 5.328E-03 & 4.817E-01 & 1.145E-03 & 8.991E-02 & 1.331E-03 & 9.091E-02 & 2.160E-03 & 1.360E-01 & 8.830E-04 & 5.903E-02 & 4.710E-04 & 2.525E-02 & 6.664E-04 & 3.349E-02 & 1.241E-03 & 5.841E-02 & 1.333E-03 & 4.733E-02 & 1.473E-03 & 4.705E-02 \\
54844.227 & 2.11 & -0.81 & 4.064E-03 & 4.809E-01 & 9.237E-04 & 9.324E-02 & 1.061E-03 & 9.228E-02 & 1.770E-03 & 1.424E-01 & 6.880E-04 & 5.882E-02 & 3.662E-04 & 2.512E-02 & 5.317E-04 & 3.403E-02 & 9.938E-04 & 5.973E-02 & 1.018E-03 & 4.536E-02 & 1.165E-03 & 4.696E-02 \\
54844.242 & 3.09 & -1.22 & 6.233E-03 & 4.722E-01 & 1.309E-03 & 8.747E-02 & 1.551E-03 & 9.080E-02 & 2.545E-03 & 1.371E-01 & 1.014E-03 & 5.830E-02 & 5.557E-04 & 2.556E-02 & 8.008E-04 & 3.453E-02 & 1.464E-03 & 5.946E-02 & 1.544E-03 & 4.711E-02 & 1.688E-03 & 4.685E-02 \\
54845.227 & 4.80 & -1.70 & 1.008E-02 & 4.605E-01 & 2.266E-03 & 9.116E-02 & 2.524E-03 & 9.027E-02 & 4.134E-03 & 1.371E-01 & 1.652E-03 & 5.877E-02 & 8.256E-04 & 2.407E-02 & 1.155E-03 & 3.183E-02 & 2.217E-03 & 5.790E-02 & 2.293E-03 & 4.613E-02 & 2.619E-03 & 4.815E-02 \\
54845.242 & 4.87 & -1.72 & 1.057E-02 & 4.681E-01 & 2.435E-03 & 9.500E-02 & 2.565E-03 & 8.990E-02 & 4.337E-03 & 1.408E-01 & 1.684E-03 & 5.903E-02 & 8.283E-04 & 2.380E-02 & 1.191E-03 & 3.221E-02 & 2.278E-03 & 5.858E-02 & 2.444E-03 & 4.817E-02 & 2.653E-03 & 4.805E-02 \\
54845.254 & 4.92 & -1.73 & 1.073E-02 & 4.679E-01 & 2.373E-03 & 9.124E-02 & 2.644E-03 & 9.106E-02 & 4.348E-03 & 1.389E-01 & 1.719E-03 & 5.925E-02 & 8.518E-04 & 2.411E-02 & 1.227E-03 & 3.240E-02 & 2.286E-03 & 5.796E-02 & 2.420E-03 & 4.727E-02 & 2.675E-03 & 4.797E-02 \\
54845.270 & 4.71 & -1.68 & 1.006E-02 & 4.649E-01 & 2.220E-03 & 9.064E-02 & 2.482E-03 & 9.043E-02 & 4.209E-03 & 1.417E-01 & 1.599E-03 & 5.862E-02 & 7.998E-04 & 2.385E-02 & 1.120E-03 & 3.147E-02 & 2.242E-03 & 5.961E-02 & 2.246E-03 & 4.612E-02 & 2.552E-03 & 4.804E-02 \\
55544.312 & 2.45 & -0.97 & 4.584E-03 & 3.933E-01 & 1.124E-03 & 8.278E-02 & 1.209E-03 & 7.881E-02 & 2.162E-03 & 1.282E-01 & 7.578E-04 & 4.862E-02 & 3.951E-04 & 2.248E-02 & 4.949E-04 & 2.714E-02 & 1.105E-03 & 5.561E-02 & 1.101E-03 & 4.194E-02 & 1.119E-03 & 3.909E-02 \\
55544.328 & 2.31 & -0.91 & 4.371E-03 & 4.055E-01 & 1.105E-03 & 8.699E-02 & 1.141E-03 & 8.003E-02 & 1.995E-03 & 1.283E-01 & 7.158E-04 & 4.936E-02 & 3.602E-04 & 2.203E-02 & 4.710E-04 & 2.729E-02 & 1.040E-03 & 5.560E-02 & 1.074E-03 & 4.333E-02 & 1.066E-03 & 3.973E-02 \\
55544.344 & 2.38 & -0.94 & 4.504E-03 & 4.055E-01 & 1.077E-03 & 8.282E-02 & 1.197E-03 & 8.075E-02 & 2.119E-03 & 1.314E-01 & 7.618E-04 & 5.103E-02 & 3.800E-04 & 2.258E-02 & 5.164E-04 & 2.899E-02 & 1.074E-03 & 5.609E-02 & 1.066E-03 & 4.174E-02 & 1.152E-03 & 4.131E-02 \\
55544.359 & 2.58 & -1.03 & 4.735E-03 & 3.928E-01 & 1.135E-03 & 8.065E-02 & 1.316E-03 & 8.159E-02 & 2.267E-03 & 1.293E-01 & 8.106E-04 & 5.005E-02 & 4.123E-04 & 2.236E-02 & 5.246E-04 & 2.733E-02 & 1.137E-03 & 5.447E-02 & 1.237E-03 & 4.416E-02 & 1.208E-03 & 3.989E-02 \\
55545.383 & 5.48 & -1.85 & 1.230E-02 & 4.152E-01 & 2.655E-03 & 7.974E-02 & 3.046E-03 & 8.220E-02 & 5.216E-03 & 1.308E-01 & 2.007E-03 & 5.448E-02 & 9.534E-04 & 2.304E-02 & 1.243E-03 & 2.920E-02 & 2.482E-03 & 5.508E-02 & 2.475E-03 & 4.361E-02 & 2.601E-03 & 4.221E-02 \\
55545.398 & 4.94 & -1.74 & 1.126E-02 & 4.286E-01 & 2.515E-03 & 8.502E-02 & 2.661E-03 & 8.074E-02 & 4.518E-03 & 1.275E-01 & 1.763E-03 & 5.379E-02 & 8.238E-04 & 2.236E-02 & 1.085E-03 & 2.857E-02 & 2.170E-03 & 5.387E-02 & 2.297E-03 & 4.474E-02 & 2.383E-03 & 4.248E-02 \\
55545.414 & 5.23 & -1.80 & 1.194E-02 & 4.244E-01 & 2.677E-03 & 8.419E-02 & 2.901E-03 & 8.218E-02 & 4.967E-03 & 1.313E-01 & 1.904E-03 & 5.459E-02 & 8.733E-04 & 2.233E-02 & 1.174E-03 & 2.910E-02 & 2.272E-03 & 5.328E-02 & 2.460E-03 & 4.514E-02 & 2.531E-03 & 4.260E-02 \\
55545.430 & 4.93 & -1.73 & 1.111E-02 & 4.234E-01 & 2.680E-03 & 8.988E-02 & 2.731E-03 & 8.289E-02 & 4.815E-03 & 1.356E-01 & 1.753E-03 & 5.376E-02 & 8.322E-04 & 2.263E-02 & 1.090E-03 & 2.875E-02 & 2.173E-03 & 5.412E-02 & 2.308E-03 & 4.489E-02 & 2.411E-03 & 4.314E-02 \\
55546.383 & 4.52 & -1.64 & 1.021E-02 & 4.194E-01 & 2.434E-03 & 8.837E-02 & 2.544E-03 & 8.316E-02 & 4.257E-03 & 1.309E-01 & 1.632E-03 & 5.413E-02 & 7.929E-04 & 2.346E-02 & 9.874E-04 & 2.844E-02 & 1.961E-03 & 5.310E-02 & 2.094E-03 & 4.462E-02 & 2.170E-03 & 4.252E-02 \\
55546.398 & 4.74 & -1.69 & 1.048E-02 & 4.159E-01 & 2.308E-03 & 8.142E-02 & 2.644E-03 & 8.294E-02 & 4.531E-03 & 1.326E-01 & 1.685E-03 & 5.382E-02 & 8.606E-04 & 2.427E-02 & 1.079E-03 & 2.956E-02 & 2.036E-03 & 5.261E-02 & 2.159E-03 & 4.392E-02 & 2.288E-03 & 4.264E-02 \\
55546.414 & 4.88 & -1.72 & 1.079E-02 & 4.129E-01 & 2.596E-03 & 8.682E-02 & 2.763E-03 & 8.331E-02 & 4.571E-03 & 1.293E-01 & 1.792E-03 & 5.467E-02 & 8.653E-04 & 2.363E-02 & 1.131E-03 & 2.994E-02 & 2.186E-03 & 5.438E-02 & 2.283E-03 & 4.443E-02 & 2.408E-03 & 4.309E-02 \\
55546.430 & 4.76 & -1.70 & 1.083E-02 & 4.259E-01 & 2.370E-03 & 8.262E-02 & 2.654E-03 & 8.234E-02 & 4.452E-03 & 1.295E-01 & 1.718E-03 & 5.431E-02 & 8.689E-04 & 2.427E-02 & 1.080E-03 & 2.947E-02 & 2.047E-03 & 5.280E-02 & 2.219E-03 & 4.467E-02 & 2.308E-03 & 4.267E-02 \\
55547.355 & 4.50 & -1.63 & 9.602E-03 & 4.235E-01 & 2.182E-03 & 8.416E-02 & 2.428E-03 & 8.310E-02 & 4.122E-03 & 1.309E-01 & 1.583E-03 & 5.501E-02 & 7.655E-04 & 2.321E-02 & 9.957E-04 & 2.947E-02 & 1.929E-03 & 5.321E-02 & 2.143E-03 & 4.492E-02 & 2.337E-03 & 4.479E-02 \\
55547.371 & 5.04 & -1.76 & 1.127E-02 & 4.301E-01 & 2.511E-03 & 8.506E-02 & 2.756E-03 & 8.320E-02 & 4.657E-03 & 1.309E-01 & 1.825E-03 & 5.599E-02 & 8.791E-04 & 2.376E-02 & 1.116E-03 & 2.935E-02 & 2.096E-03 & 5.184E-02 & 2.416E-03 & 4.546E-02 & 2.498E-03 & 4.313E-02 \\
55547.387 & 5.76 & -1.90 & 1.315E-02 & 4.280E-01 & 3.115E-03 & 8.914E-02 & 3.243E-03 & 8.406E-02 & 5.529E-03 & 1.335E-01 & 2.067E-03 & 5.501E-02 & 1.016E-03 & 2.375E-02 & 1.343E-03 & 3.068E-02 & 2.509E-03 & 5.401E-02 & 2.719E-03 & 4.526E-02 & 2.942E-03 & 4.473E-02 \\
55547.402 & 5.79 & -1.91 & 1.333E-02 & 4.311E-01 & 3.043E-03 & 8.687E-02 & 3.283E-03 & 8.475E-02 & 5.416E-03 & 1.302E-01 & 2.123E-03 & 5.575E-02 & 1.069E-03 & 2.476E-02 & 1.314E-03 & 2.987E-02 & 2.569E-03 & 5.469E-02 & 2.733E-03 & 4.504E-02 & 2.930E-03 & 4.420E-02 \\
55548.348 & 3.50 & -1.36 & 7.598E-03 & 4.471E-01 & 1.617E-03 & 8.402E-02 & 1.882E-03 & 8.490E-02 & 3.201E-03 & 1.346E-01 & 1.198E-03 & 5.530E-02 & 6.182E-04 & 2.435E-02 & 8.022E-04 & 3.055E-02 & 1.579E-03 & 5.655E-02 & 1.557E-03 & 4.217E-02 & 1.788E-03 & 4.399E-02 \\
55548.363 & 4.01 & -1.51 & 8.432E-03 & 4.297E-01 & 1.968E-03 & 8.766E-02 & 2.175E-03 & 8.542E-02 & 3.614E-03 & 1.317E-01 & 1.413E-03 & 5.607E-02 & 7.450E-04 & 2.542E-02 & 8.722E-04 & 2.889E-02 & 1.818E-03 & 5.686E-02 & 1.902E-03 & 4.472E-02 & 1.953E-03 & 4.208E-02 \\
55548.379 & 4.33 & -1.59 & 9.164E-03 & 4.253E-01 & 2.108E-03 & 8.533E-02 & 2.362E-03 & 8.480E-02 & 3.995E-03 & 1.328E-01 & 1.538E-03 & 5.559E-02 & 7.833E-04 & 2.446E-02 & 9.531E-04 & 2.892E-02 & 1.920E-03 & 5.544E-02 & 1.947E-03 & 4.268E-02 & 2.150E-03 & 4.283E-02 \\
55548.395 & 4.77 & -1.70 & 1.020E-02 & 4.236E-01 & 2.206E-03 & 8.122E-02 & 2.608E-03 & 8.472E-02 & 4.488E-03 & 1.351E-01 & 1.683E-03 & 5.540E-02 & 8.151E-04 & 2.321E-02 & 1.138E-03 & 3.107E-02 & 2.148E-03 & 5.611E-02 & 2.199E-03 & 4.372E-02 & 2.298E-03 & 4.195E-02 \\
55549.316 & 1.24 & -0.24 & 3.307E-03 & 2.872E-01 & 7.995E-04 & 6.902E-02 & 5.049E-04 & 4.408E-02 & 1.244E-03 & 1.074E-01 & 2.056E-04 & 1.937E-02 & 2.430E-04 & 2.231E-02 & 2.388E-04 & 2.261E-02 & 3.693E-04 & 3.352E-02 & 4.792E-04 & 3.868E-02 & 5.272E-04 & 4.010E-02 \\
55549.332 & 2.76 & -1.10 & 6.197E-03 & 3.762E-01 & 1.411E-03 & 7.880E-02 & 1.363E-03 & 6.955E-02 & 2.504E-03 & 1.222E-01 & 8.279E-04 & 4.402E-02 & 5.144E-04 & 2.449E-02 & 6.230E-04 & 2.916E-02 & 1.149E-03 & 5.092E-02 & 1.220E-03 & 4.180E-02 & 1.236E-03 & 3.879E-02 \\
55549.348 & 2.66 & -1.06 & 6.034E-03 & 3.741E-01 & 1.274E-03 & 7.319E-02 & 1.364E-03 & 7.273E-02 & 2.424E-03 & 1.218E-01 & 8.141E-04 & 4.488E-02 & 5.026E-04 & 2.487E-02 & 5.926E-04 & 2.872E-02 & 1.161E-03 & 5.319E-02 & 1.130E-03 & 4.037E-02 & 1.270E-03 & 4.152E-02 \\
55549.363 & 2.75 & -1.10 & 6.155E-03 & 3.842E-01 & 1.470E-03 & 8.393E-02 & 1.393E-03 & 7.310E-02 & 2.405E-03 & 1.194E-01 & 8.380E-04 & 4.527E-02 & 5.289E-04 & 2.542E-02 & 6.009E-04 & 2.844E-02 & 1.173E-03 & 5.199E-02 & 1.184E-03 & 4.096E-02 & 1.287E-03 & 4.064E-02 \\
55554.410 & 2.64 & -1.05 & 3.864E-03 & 2.836E-01 & 1.005E-03 & 6.441E-02 & 1.086E-03 & 6.342E-02 & 1.839E-03 & 9.983E-02 & 7.306E-04 & 4.265E-02 & 3.824E-04 & 2.000E-02 & 4.707E-04 & 2.393E-02 & 8.769E-04 & 4.180E-02 & 1.020E-03 & 3.602E-02 & 9.859E-04 & 3.258E-02 \\
55554.426 & 2.74 & -1.09 & 3.812E-03 & 2.772E-01 & 1.143E-03 & 7.245E-02 & 1.123E-03 & 6.448E-02 & 1.878E-03 & 9.914E-02 & 7.681E-04 & 4.345E-02 & 3.779E-04 & 1.939E-02 & 5.353E-04 & 2.622E-02 & 9.519E-04 & 4.330E-02 & 1.055E-03 & 3.611E-02 & 1.049E-03 & 3.306E-02 \\
55554.445 & 2.30 & -0.91 & 3.383E-03 & 2.945E-01 & 1.054E-03 & 7.845E-02 & 9.779E-04 & 6.710E-02 & 1.659E-03 & 1.050E-01 & 6.705E-04 & 4.495E-02 & 3.247E-04 & 1.969E-02 & 4.303E-04 & 2.502E-02 & 8.016E-04 & 4.317E-02 & 8.988E-04 & 3.633E-02 & 8.462E-04 & 3.190E-02 \\
55555.312 & 4.03 & -1.51 & 6.833E-03 & 3.077E-01 & 1.649E-03 & 6.682E-02 & 1.777E-03 & 6.597E-02 & 3.081E-03 & 1.063E-01 & 1.194E-03 & 4.466E-02 & 5.584E-04 & 1.887E-02 & 7.803E-04 & 2.539E-02 & 1.477E-03 & 4.506E-02 & 1.648E-03 & 3.871E-02 & 1.530E-03 & 3.371E-02 \\
55555.328 & 3.64 & -1.40 & 6.090E-03 & 3.096E-01 & 1.558E-03 & 7.040E-02 & 1.643E-03 & 6.763E-02 & 2.854E-03 & 1.095E-01 & 1.092E-03 & 4.524E-02 & 4.919E-04 & 1.848E-02 & 6.846E-04 & 2.512E-02 & 1.350E-03 & 4.605E-02 & 1.448E-03 & 3.776E-02 & 1.414E-03 & 3.412E-02 \\
55555.348 & 4.10 & -1.53 & 6.958E-03 & 3.112E-01 & 1.718E-03 & 6.889E-02 & 1.907E-03 & 6.966E-02 & 3.188E-03 & 1.085E-01 & 1.233E-03 & 4.524E-02 & 6.113E-04 & 2.032E-02 & 7.633E-04 & 2.470E-02 & 1.494E-03 & 4.510E-02 & 1.554E-03 & 3.642E-02 & 1.626E-03 & 3.519E-02 \\
55555.363 & 3.96 & -1.50 & 6.892E-03 & 3.162E-01 & 1.534E-03 & 6.390E-02 & 1.858E-03 & 6.990E-02 & 3.146E-03 & 1.106E-01 & 1.211E-03 & 4.597E-02 & 5.604E-04 & 1.931E-02 & 7.234E-04 & 2.441E-02 & 1.464E-03 & 4.577E-02 & 1.538E-03 & 3.716E-02 & 1.632E-03 & 3.617E-02 \\
55560.316 & 0.53 & 0.68 & 5.610E-04 & 3.278E-01 & 1.500E-04 & 7.469E-02 & 1.583E-04 & 6.562E-02 & 4.199E-04 & 1.391E-01 & 9.526E-05 & 3.377E-02 & 5.468E-05 & 1.590E-02 & 7.216E-05 & 1.928E-02 & 2.161E-04 & 5.282E-02 & 1.770E-04 & 2.886E-02 & 1.818E-04 & 2.735E-02 \\
55560.332 & 0.45 & 0.86 & 2.505E-04 & 1.880E-01 & 9.620E-05 & 5.510E-02 & 1.578E-04 & 7.340E-02 & 3.521E-04 & 1.392E-01 & 7.478E-05 & 3.277E-02 & 4.962E-05 & 1.698E-02 & 6.820E-05 & 2.161E-02 & 1.683E-04 & 4.840E-02 & 1.770E-04 & 3.325E-02 & 1.742E-04 & 2.979E-02 \\
55560.348 & 0.33 & 1.20 & 2.337E-04 & 2.356E-01 & 6.955E-05 & 5.720E-02 & 8.832E-05 & 6.203E-02 & 2.153E-04 & 1.241E-01 & 4.310E-05 & 2.559E-02 & 3.015E-05 & 1.535E-02 & 4.629E-05 & 1.996E-02 & 1.316E-04 & 5.367E-02 & 1.187E-04 & 3.103E-02 & 1.320E-04 & 3.212E-02 \\
55560.363 & 0.36 & 1.11 & 4.134E-04 & 3.946E-01 & 7.164E-05 & 6.013E-02 & 1.445E-04 & 8.599E-02 & 3.625E-04 & 1.519E-01 & 5.136E-05 & 2.781E-02 & 2.837E-05 & 1.303E-02 & 5.120E-05 & 2.015E-02 & 1.657E-04 & 6.033E-02 & 1.456E-04 & 3.394E-02 & 1.325E-04 & 2.838E-02 \\
56255.426 & 0.05 & 3.17 & 5.699E-05 & 3.687E-01 & 1.675E-05 & 9.318E-02 & 1.691E-05 & 7.547E-02 & 2.959E-05 & 1.209E-01 & 1.294E-05 & 5.178E-02 & 7.740E-06 & 2.455E-02 & 1.115E-05 & 2.982E-02 & 2.240E-05 & 5.542E-02 & 2.683E-05 & 4.225E-02 & 3.026E-05 & 4.264E-02 \\
56255.441 & 0.08 & 2.70 & 7.319E-05 & 3.712E-01 & 2.347E-05 & 9.584E-02 & 2.600E-05 & 8.248E-02 & 4.402E-05 & 1.249E-01 & 2.285E-05 & 4.933E-02 & 1.105E-05 & 2.318E-02 & 1.664E-05 & 2.948E-02 & 3.279E-05 & 5.305E-02 & 4.495E-05 & 4.380E-02 & 5.498E-05 & 4.805E-02 \\
56255.461 & 0.14 & 2.12 & 1.278E-04 & 4.411E-01 & 3.380E-05 & 8.876E-02 & 4.111E-05 & 8.397E-02 & 8.045E-05 & 1.375E-01 & 3.121E-05 & 5.302E-02 & 1.970E-05 & 2.463E-02 & 3.123E-05 & 3.247E-02 & 5.784E-05 & 5.577E-02 & 8.000E-05 & 4.541E-02 & 8.840E-05 & 4.530E-02 \\
56255.477 & 0.17 & 1.94 & 1.461E-04 & 4.300E-01 & 4.025E-05 & 9.050E-02 & 5.117E-05 & 8.482E-02 & 9.729E-05 & 1.408E-01 & 3.585E-05 & 5.132E-02 & 2.219E-05 & 2.356E-02 & 3.740E-05 & 3.274E-02 & 6.811E-05 & 5.601E-02 & 9.099E-05 & 4.361E-02 & 1.050E-04 & 4.543E-02 \\
56255.492 & 0.16 & 1.96 & 1.474E-04 & 4.275E-01 & 4.355E-05 & 9.904E-02 & 5.220E-05 & 8.887E-02 & 9.731E-05 & 1.413E-01 & 3.750E-05 & 5.446E-02 & 2.407E-05 & 2.571E-02 & 3.428E-05 & 3.104E-02 & 6.776E-05 & 5.614E-02 & 8.924E-05 & 4.407E-02 & 1.056E-04 & 4.673E-02 \\
56255.504 & 0.17 & 1.92 & 1.465E-04 & 4.192E-01 & 4.209E-05 & 9.369E-02 & 5.510E-05 & 9.119E-02 & 9.679E-05 & 1.379E-01 & 3.855E-05 & 5.432E-02 & 2.093E-05 & 2.170E-02 & 3.601E-05 & 3.128E-02 & 7.370E-05 & 5.795E-02 & 9.636E-05 & 4.548E-02 & 1.073E-04 & 4.586E-02 \\
56256.445 & 0.13 & 2.22 & 1.282E-04 & 4.028E-01 & 3.416E-05 & 8.594E-02 & 3.999E-05 & 7.747E-02 & 6.984E-05 & 1.201E-01 & 2.839E-05 & 4.810E-02 & 1.891E-05 & 2.392E-02 & 2.547E-05 & 2.857E-02 & 5.514E-05 & 5.669E-02 & 7.383E-05 & 4.725E-02 & 8.368E-05 & 4.902E-02 \\
56256.461 & 0.09 & 2.63 & 1.069E-04 & 4.079E-01 & 2.906E-05 & 9.394E-02 & 2.920E-05 & 7.485E-02 & 5.616E-05 & 1.301E-01 & 1.880E-05 & 4.140E-02 & 1.267E-05 & 2.303E-02 & 2.094E-05 & 3.281E-02 & 3.509E-05 & 5.186E-02 & 4.324E-05 & 4.148E-02 & 5.313E-05 & 4.642E-02 \\
56256.477 & 0.16 & 2.01 & 1.616E-04 & 4.372E-01 & 3.961E-05 & 8.748E-02 & 5.201E-05 & 8.603E-02 & 8.829E-05 & 1.298E-01 & 3.642E-05 & 5.120E-02 & 2.431E-05 & 2.575E-02 & 3.402E-05 & 3.084E-02 & 7.157E-05 & 6.061E-02 & 9.561E-05 & 4.941E-02 & 9.964E-05 & 4.764E-02 \\
56256.492 & 0.12 & 2.29 & 1.206E-04 & 4.079E-01 & 3.209E-05 & 8.819E-02 & 3.820E-05 & 8.058E-02 & 7.397E-05 & 1.374E-01 & 2.788E-05 & 5.159E-02 & 2.004E-05 & 2.739E-02 & 2.468E-05 & 2.989E-02 & 4.916E-05 & 5.503E-02 & 6.837E-05 & 4.683E-02 & 7.646E-05 & 4.764E-02 \\
56257.535 & 0.16 & 1.97 & 1.819E-04 & 3.967E-01 & 3.857E-05 & 7.265E-02 & 4.948E-05 & 7.184E-02 & 9.978E-05 & 1.295E-01 & 3.623E-05 & 4.619E-02 & 2.135E-05 & 2.159E-02 & 3.324E-05 & 2.883E-02 & 7.131E-05 & 5.727E-02 & 1.001E-04 & 4.955E-02 & 9.612E-05 & 4.552E-02 \\
56257.551 & 0.07 & 2.93 & 9.976E-05 & 3.335E-01 & 2.422E-05 & 7.591E-02 & 1.718E-05 & 4.757E-02 & 4.012E-05 & 1.043E-01 & 1.146E-05 & 2.890E-02 & 8.590E-06 & 1.892E-02 & 1.109E-05 & 2.206E-02 & 2.227E-05 & 4.097E-02 & 3.344E-05 & 4.355E-02 & 3.383E-05 & 4.187E-02 \\
56257.566 & 0.02 & 4.12 & 2.769E-05 & 1.621E-01 & 8.140E-06 & 4.738E-02 & 7.400E-07 & 4.280E-03 & 1.187E-05 & 6.229E-02 & 1.360E-06 & 6.916E-03 & 3.810E-06 & 1.942E-02 & 3.110E-06 & 1.546E-02 & 2.850E-06 & 1.372E-02 & 1.020E-05 & 4.353E-02 & 7.750E-06 & 3.524E-02 \\
56257.582 & 0.02 & 4.38 & 3.880E-05 & 2.474E-01 & 9.650E-06 & 6.127E-02 & 3.450E-06 & 2.302E-02 & 1.120E-05 & 7.351E-02 & 1.900E-07 & 1.261E-03 & 2.690E-06 & 1.618E-02 & 3.270E-06 & 1.944E-02 & 7.900E-07 & 4.775E-03 & 6.300E-06 & 3.695E-02 & 7.990E-06 & 4.775E-02 \\
56258.410 & 0.18 & 1.85 & 2.227E-04 & 3.688E-01 & 4.728E-05 & 6.893E-02 & 5.665E-05 & 6.739E-02 & 1.279E-04 & 1.278E-01 & 3.849E-05 & 4.091E-02 & 2.705E-05 & 2.320E-02 & 3.493E-05 & 2.646E-02 & 8.349E-05 & 5.830E-02 & 9.571E-05 & 4.482E-02 & 1.115E-04 & 4.845E-02 \\
56258.426 & 0.16 & 1.96 & 2.033E-04 & 3.744E-01 & 4.501E-05 & 7.225E-02 & 4.994E-05 & 6.587E-02 & 1.071E-04 & 1.259E-01 & 3.443E-05 & 4.069E-02 & 2.392E-05 & 2.282E-02 & 3.270E-05 & 2.765E-02 & 7.364E-05 & 5.683E-02 & 8.460E-05 & 4.394E-02 & 9.208E-05 & 4.452E-02 \\
56258.441 & 0.22 & 1.66 & 2.476E-04 & 3.950E-01 & 5.552E-05 & 7.648E-02 & 6.522E-05 & 7.026E-02 & 1.429E-04 & 1.347E-01 & 5.063E-05 & 4.699E-02 & 3.308E-05 & 2.449E-02 & 4.301E-05 & 2.776E-02 & 1.031E-04 & 6.071E-02 & 1.177E-04 & 4.561E-02 & 1.311E-04 & 4.716E-02 \\
56258.457 & 0.16 & 1.98 & 2.295E-04 & 3.414E-01 & 4.918E-05 & 6.780E-02 & 5.080E-05 & 5.895E-02 & 1.084E-04 & 1.168E-01 & 2.983E-05 & 3.208E-02 & 2.552E-05 & 2.296E-02 & 3.164E-05 & 2.570E-02 & 6.585E-05 & 4.992E-02 & 8.031E-05 & 4.330E-02 & 9.428E-05 & 4.750E-02 \\
56259.422 & 0.22 & 1.64 & 3.048E-04 & 3.617E-01 & 7.438E-05 & 8.056E-02 & 6.974E-05 & 6.401E-02 & 1.503E-04 & 1.244E-01 & 4.735E-05 & 3.962E-02 & 2.990E-05 & 2.070E-02 & 4.418E-05 & 2.724E-02 & 1.000E-04 & 5.756E-02 & 1.164E-04 & 4.491E-02 & 1.277E-04 & 4.644E-02 \\
56259.438 & 0.23 & 1.61 & 2.814E-04 & 3.621E-01 & 7.018E-05 & 8.120E-02 & 6.946E-05 & 6.768E-02 & 1.439E-04 & 1.246E-01 & 4.944E-05 & 4.255E-02 & 3.428E-05 & 2.376E-02 & 4.469E-05 & 2.734E-02 & 1.044E-04 & 6.005E-02 & 1.204E-04 & 4.538E-02 & 1.383E-04 & 4.784E-02 \\
56259.449 & 0.23 & 1.61 & 2.671E-04 & 3.761E-01 & 6.756E-05 & 8.240E-02 & 7.745E-05 & 7.641E-02 & 1.444E-04 & 1.257E-01 & 5.239E-05 & 4.640E-02 & 3.174E-05 & 2.226E-02 & 4.828E-05 & 2.957E-02 & 1.110E-04 & 6.298E-02 & 1.233E-04 & 4.552E-02 & 1.394E-04 & 4.771E-02 \\
56259.465 & 0.23 & 1.61 & 2.732E-04 & 3.814E-01 & 6.663E-05 & 8.047E-02 & 7.675E-05 & 7.618E-02 & 1.438E-04 & 1.290E-01 & 5.112E-05 & 4.605E-02 & 2.966E-05 & 2.119E-02 & 4.528E-05 & 2.803E-02 & 1.136E-04 & 6.410E-02 & 1.337E-04 & 4.858E-02 & 1.370E-04 & 4.738E-02 \\
56260.273 & 0.14 & 2.17 & 1.731E-04 & 3.383E-01 & 4.230E-05 & 7.655E-02 & 3.450E-05 & 5.644E-02 & 7.948E-05 & 1.176E-01 & 2.401E-05 & 3.507E-02 & 1.840E-05 & 2.135E-02 & 2.948E-05 & 2.926E-02 & 5.696E-05 & 5.319E-02 & 7.349E-05 & 4.647E-02 & 8.307E-05 & 4.868E-02 \\
56260.289 & 0.15 & 2.07 & 1.801E-04 & 3.550E-01 & 4.122E-05 & 7.705E-02 & 3.715E-05 & 6.016E-02 & 8.247E-05 & 1.184E-01 & 2.638E-05 & 3.757E-02 & 2.161E-05 & 2.340E-02 & 2.814E-05 & 2.645E-02 & 6.689E-05 & 5.713E-02 & 7.481E-05 & 4.387E-02 & 9.425E-05 & 5.055E-02 \\
56260.305 & 0.16 & 1.97 & 1.823E-04 & 3.625E-01 & 3.986E-05 & 7.083E-02 & 4.474E-05 & 6.658E-02 & 8.533E-05 & 1.140E-01 & 3.109E-05 & 4.064E-02 & 2.387E-05 & 2.431E-02 & 3.063E-05 & 2.686E-02 & 7.285E-05 & 5.711E-02 & 9.136E-05 & 4.794E-02 & 1.020E-04 & 4.881E-02 \\
56260.320 & 0.17 & 1.91 & 1.819E-04 & 3.621E-01 & 4.467E-05 & 7.678E-02 & 4.738E-05 & 6.730E-02 & 1.023E-04 & 1.305E-01 & 3.433E-05 & 4.342E-02 & 2.586E-05 & 2.480E-02 & 3.619E-05 & 2.896E-02 & 8.013E-05 & 5.926E-02 & 8.707E-05 & 4.336E-02 & 1.077E-04 & 4.878E-02 \\
56261.355 & 0.14 & 2.11 & 1.552E-04 & 3.656E-01 & 4.229E-05 & 8.686E-02 & 4.234E-05 & 6.933E-02 & 8.237E-05 & 1.229E-01 & 3.084E-05 & 4.413E-02 & 2.387E-05 & 2.710E-02 & 2.932E-05 & 2.816E-02 & 6.731E-05 & 5.870E-02 & 7.472E-05 & 4.352E-02 & 8.643E-05 & 4.609E-02 \\
56261.367 & 0.17 & 1.96 & 1.857E-04 & 3.713E-01 & 4.951E-05 & 8.542E-02 & 4.793E-05 & 6.691E-02 & 9.645E-05 & 1.226E-01 & 3.294E-05 & 4.073E-02 & 2.698E-05 & 2.577E-02 & 3.427E-05 & 2.819E-02 & 7.030E-05 & 5.389E-02 & 8.793E-05 & 4.448E-02 & 9.712E-05 & 4.559E-02 \\
56261.383 & 0.10 & 2.46 & 1.842E-04 & 2.919E-01 & 3.788E-05 & 5.504E-02 & 2.606E-05 & 3.620E-02 & 6.471E-05 & 8.889E-02 & 9.050E-06 & 1.224E-02 & 2.051E-05 & 2.463E-02 & 1.781E-05 & 2.031E-02 & 3.164E-05 & 3.426E-02 & 3.799E-05 & 3.471E-02 & 5.314E-05 & 4.617E-02 \\
56261.398 & 0.05 & 3.16 & 1.254E-04 & 2.590E-01 & 2.357E-05 & 4.930E-02 & 1.130E-05 & 2.303E-02 & 3.277E-05 & 6.847E-02 & 1.570E-06 & 3.153E-03 & 1.004E-05 & 2.024E-02 & 8.070E-06 & 1.541E-02 & 1.159E-05 & 2.137E-02 & 1.244E-05 & 2.445E-02 & 2.260E-05 & 4.352E-02 \\
56262.473 & 0.14 & 2.16 & 1.364E-04 & 4.132E-01 & 3.524E-05 & 8.888E-02 & 3.922E-05 & 7.772E-02 & 7.371E-05 & 1.267E-01 & 2.875E-05 & 4.824E-02 & 1.864E-05 & 2.357E-02 & 2.589E-05 & 2.705E-02 & 6.054E-05 & 5.796E-02 & 7.545E-05 & 4.494E-02 & 8.623E-05 & 4.695E-02 \\
56262.488 & 0.15 & 2.02 & 1.364E-04 & 3.967E-01 & 3.757E-05 & 8.912E-02 & 4.424E-05 & 8.072E-02 & 8.426E-05 & 1.305E-01 & 3.146E-05 & 4.863E-02 & 2.031E-05 & 2.299E-02 & 3.246E-05 & 3.048E-02 & 6.880E-05 & 5.948E-02 & 8.667E-05 & 4.569E-02 & 1.011E-04 & 4.878E-02 \\
56262.504 & 0.15 & 2.07 & 1.236E-04 & 3.762E-01 & 3.201E-05 & 7.922E-02 & 4.146E-05 & 7.748E-02 & 8.199E-05 & 1.325E-01 & 3.093E-05 & 4.965E-02 & 2.340E-05 & 2.706E-02 & 3.075E-05 & 2.986E-02 & 6.633E-05 & 5.917E-02 & 7.900E-05 & 4.333E-02 & 9.928E-05 & 4.841E-02 \\
56262.520 & 0.03 & 3.69 & 7.295E-05 & 2.656E-01 & 1.616E-05 & 5.871E-02 & 5.990E-06 & 2.081E-02 & 2.045E-05 & 7.201E-02 & 7.000E-07 & 2.464E-03 & 7.500E-06 & 2.477E-02 & 4.670E-06 & 1.511E-02 & 1.870E-06 & 5.968E-03 & 1.119E-05 & 3.434E-02 & 1.514E-05 & 4.780E-02 \\
56263.426 & 0.11 & 2.43 & 1.061E-04 & 4.248E-01 & 2.968E-05 & 9.990E-02 & 3.156E-05 & 8.084E-02 & 5.860E-05 & 1.313E-01 & 2.318E-05 & 5.094E-02 & 1.766E-05 & 2.884E-02 & 2.290E-05 & 3.109E-02 & 4.972E-05 & 6.155E-02 & 5.704E-05 & 4.353E-02 & 6.586E-05 & 4.543E-02 \\
56263.441 & 0.13 & 2.24 & 1.128E-04 & 4.137E-01 & 3.004E-05 & 9.028E-02 & 3.711E-05 & 8.282E-02 & 6.681E-05 & 1.317E-01 & 2.612E-05 & 5.024E-02 & 2.105E-05 & 2.925E-02 & 3.034E-05 & 3.463E-02 & 5.534E-05 & 5.940E-02 & 7.461E-05 & 4.738E-02 & 8.371E-05 & 4.786E-02 \\
56263.457 & 0.14 & 2.15 & 1.179E-04 & 4.036E-01 & 2.666E-05 & 7.376E-02 & 3.957E-05 & 8.199E-02 & 7.842E-05 & 1.368E-01 & 2.775E-05 & 4.896E-02 & 2.087E-05 & 2.672E-02 & 3.102E-05 & 3.261E-02 & 6.567E-05 & 6.342E-02 & 7.478E-05 & 4.357E-02 & 8.802E-05 & 4.621E-02 \\
56263.473 & 0.08 & 2.81 & 7.934E-05 & 3.725E-01 & 1.987E-05 & 8.494E-02 & 2.124E-05 & 7.091E-02 & 4.326E-05 & 1.267E-01 & 1.469E-05 & 4.253E-02 & 1.315E-05 & 2.942E-02 & 1.550E-05 & 2.968E-02 & 3.273E-05 & 5.683E-02 & 4.102E-05 & 4.528E-02 & 4.565E-05 & 4.580E-02 \\
56265.492 & 0.20 & 1.73 & 1.635E-04 & 4.246E-01 & 4.600E-05 & 9.013E-02 & 5.878E-05 & 8.544E-02 & 1.160E-04 & 1.369E-01 & 4.523E-05 & 5.443E-02 & 3.177E-05 & 2.736E-02 & 4.571E-05 & 3.260E-02 & 9.802E-05 & 6.325E-02 & 1.210E-04 & 4.739E-02 & 1.284E-04 & 4.631E-02 \\
56265.508 & 0.19 & 1.83 & 1.556E-04 & 4.328E-01 & 4.507E-05 & 9.923E-02 & 5.887E-05 & 8.852E-02 & 1.126E-04 & 1.518E-01 & 3.863E-05 & 5.153E-02 & 2.467E-05 & 2.417E-02 & 4.037E-05 & 3.234E-02 & 8.370E-05 & 6.055E-02 & 1.050E-04 & 4.586E-02 & 1.203E-04 & 4.719E-02 \\
56265.523 & 0.18 & 1.88 & 1.509E-04 & 4.478E-01 & 4.302E-05 & 9.578E-02 & 4.963E-05 & 8.485E-02 & 9.554E-05 & 1.377E-01 & 3.800E-05 & 5.316E-02 & 2.377E-05 & 2.396E-02 & 3.748E-05 & 3.131E-02 & 8.748E-05 & 6.502E-02 & 9.812E-05 & 4.492E-02 & 1.201E-04 & 4.941E-02 \\
56265.535 & 0.17 & 1.92 & 1.430E-04 & 4.580E-01 & 4.173E-05 & 9.938E-02 & 4.904E-05 & 8.668E-02 & 9.630E-05 & 1.435E-01 & 3.566E-05 & 5.297E-02 & 2.391E-05 & 2.532E-02 & 3.678E-05 & 3.218E-02 & 8.102E-05 & 6.294E-02 & 9.861E-05 & 4.644E-02 & 1.127E-04 & 4.840E-02 \\
56268.371 & 0.19 & 1.79 & 1.706E-04 & 4.451E-01 & 4.514E-05 & 8.990E-02 & 5.989E-05 & 8.820E-02 & 1.094E-04 & 1.386E-01 & 4.415E-05 & 5.387E-02 & 2.886E-05 & 2.654E-02 & 4.478E-05 & 3.356E-02 & 9.117E-05 & 6.273E-02 & 1.081E-04 & 4.583E-02 & 1.244E-04 & 4.793E-02 \\
56268.387 & 0.20 & 1.73 & 1.849E-04 & 4.597E-01 & 5.237E-05 & 9.780E-02 & 6.454E-05 & 8.839E-02 & 1.238E-04 & 1.462E-01 & 4.947E-05 & 5.671E-02 & 3.011E-05 & 2.618E-02 & 4.704E-05 & 3.323E-02 & 9.888E-05 & 6.327E-02 & 1.145E-04 & 4.575E-02 & 1.311E-04 & 4.777E-02 \\
56268.402 & 0.14 & 2.10 & 1.399E-04 & 4.826E-01 & 4.292E-05 & 1.109E-01 & 4.394E-05 & 8.622E-02 & 8.907E-05 & 1.468E-01 & 3.547E-05 & 5.591E-02 & 2.316E-05 & 2.813E-02 & 3.260E-05 & 3.202E-02 & 6.968E-05 & 6.256E-02 & 8.557E-05 & 4.765E-02 & 9.718E-05 & 4.923E-02 \\
56268.418 & 0.17 & 1.92 & 1.549E-04 & 4.692E-01 & 3.548E-05 & 8.357E-02 & 5.222E-05 & 8.865E-02 & 9.523E-05 & 1.380E-01 & 4.065E-05 & 5.644E-02 & 2.585E-05 & 2.695E-02 & 3.788E-05 & 3.253E-02 & 8.416E-05 & 6.439E-02 & 1.040E-04 & 4.873E-02 & 1.094E-04 & 4.710E-02 \\
56269.441 & 0.16 & 2.01 & 1.420E-04 & 4.556E-01 & 3.794E-05 & 9.456E-02 & 4.926E-05 & 8.993E-02 & 9.179E-05 & 1.432E-01 & 3.347E-05 & 5.212E-02 & 2.545E-05 & 2.845E-02 & 3.099E-05 & 2.873E-02 & 7.693E-05 & 6.441E-02 & 9.000E-05 & 4.626E-02 & 1.006E-04 & 4.716E-02 \\
56269.457 & 0.17 & 1.93 & 1.416E-04 & 4.333E-01 & 4.064E-05 & 9.367E-02 & 5.242E-05 & 8.915E-02 & 9.583E-05 & 1.392E-01 & 4.280E-05 & 5.535E-02 & 2.502E-05 & 2.578E-02 & 3.716E-05 & 3.177E-02 & 8.041E-05 & 6.332E-02 & 9.668E-05 & 4.660E-02 & 1.110E-04 & 4.840E-02 \\
56269.473 & 0.18 & 1.89 & 1.546E-04 & 4.490E-01 & 4.065E-05 & 9.108E-02 & 5.038E-05 & 8.347E-02 & 9.614E-05 & 1.352E-01 & 3.936E-05 & 5.375E-02 & 2.539E-05 & 2.551E-02 & 3.842E-05 & 3.173E-02 & 8.416E-05 & 6.267E-02 & 1.006E-04 & 4.633E-02 & 1.164E-04 & 4.869E-02 \\
56269.488 & 0.17 & 1.90 & 1.555E-04 & 4.573E-01 & 4.487E-05 & 9.906E-02 & 5.086E-05 & 8.543E-02 & 9.892E-05 & 1.420E-01 & 3.974E-05 & 5.488E-02 & 2.671E-05 & 2.696E-02 & 3.828E-05 & 3.200E-02 & 8.024E-05 & 6.174E-02 & 9.622E-05 & 4.488E-02 & 1.088E-04 & 4.576E-02 \\
56270.418 & 0.11 & 2.35 & 1.021E-04 & 4.573E-01 & 2.262E-05 & 8.381E-02 & 3.213E-05 & 8.397E-02 & 6.480E-05 & 1.450E-01 & 2.412E-05 & 5.312E-02 & 1.464E-05 & 2.331E-02 & 2.265E-05 & 2.959E-02 & 5.042E-05 & 6.023E-02 & 6.522E-05 & 4.550E-02 & 7.350E-05 & 4.628E-02 \\
56270.430 & 0.13 & 2.25 & 9.969E-05 & 4.243E-01 & 3.194E-05 & 1.058E-01 & 3.827E-05 & 9.289E-02 & 7.063E-05 & 1.419E-01 & 2.663E-05 & 5.393E-02 & 1.711E-05 & 2.461E-02 & 2.545E-05 & 3.037E-02 & 5.580E-05 & 6.120E-02 & 6.822E-05 & 4.407E-02 & 8.560E-05 & 4.903E-02 \\
56270.445 & 0.13 & 2.22 & 9.720E-05 & 4.042E-01 & 2.943E-05 & 9.406E-02 & 3.693E-05 & 8.691E-02 & 7.010E-05 & 1.406E-01 & 2.701E-05 & 5.314E-02 & 1.556E-05 & 2.230E-02 & 2.815E-05 & 3.257E-02 & 6.093E-05 & 6.409E-02 & 7.456E-05 & 4.613E-02 & 8.683E-05 & 4.854E-02 \\
56270.461 & 0.14 & 2.15 & 1.196E-04 & 4.731E-01 & 3.261E-05 & 9.785E-02 & 3.909E-05 & 8.592E-02 & 7.419E-05 & 1.383E-01 & 3.163E-05 & 5.804E-02 & 1.329E-05 & 1.799E-02 & 2.779E-05 & 3.043E-02 & 6.176E-05 & 6.128E-02 & 8.008E-05 & 4.621E-02 & 9.039E-05 & 4.739E-02 \\
56271.352 & 0.16 & 2.02 & 1.185E-04 & 4.201E-01 & 3.471E-05 & 9.143E-02 & 4.575E-05 & 8.915E-02 & 8.562E-05 & 1.410E-01 & 3.215E-05 & 5.300E-02 & 1.830E-05 & 2.151E-02 & 3.392E-05 & 3.270E-02 & 6.925E-05 & 6.143E-02 & 8.609E-05 & 4.508E-02 & 9.751E-05 & 4.623E-02 \\
56271.367 & 0.16 & 1.99 & 1.298E-04 & 4.383E-01 & 3.881E-05 & 9.929E-02 & 4.628E-05 & 8.869E-02 & 9.251E-05 & 1.477E-01 & 3.705E-05 & 5.763E-02 & 1.753E-05 & 2.034E-02 & 3.287E-05 & 3.057E-02 & 6.832E-05 & 5.991E-02 & 9.161E-05 & 4.630E-02 & 1.024E-04 & 4.699E-02 \\
56271.383 & 0.16 & 1.99 & 1.297E-04 & 4.403E-01 & 3.730E-05 & 9.699E-02 & 4.761E-05 & 9.002E-02 & 8.447E-05 & 1.360E-01 & 3.440E-05 & 5.437E-02 & 1.920E-05 & 2.193E-02 & 3.582E-05 & 3.296E-02 & 7.054E-05 & 6.087E-02 & 8.777E-05 & 4.452E-02 & 1.001E-04 & 4.557E-02 \\
56271.395 & 0.15 & 2.04 & 1.248E-04 & 4.505E-01 & 3.881E-05 & 1.052E-01 & 4.293E-05 & 8.706E-02 & 8.273E-05 & 1.407E-01 & 3.129E-05 & 5.312E-02 & 1.840E-05 & 2.174E-02 & 3.089E-05 & 3.051E-02 & 7.004E-05 & 6.321E-02 & 8.556E-05 & 4.527E-02 & 9.524E-05 & 4.560E-02 \\
57011.402 & 0.22 & 1.65 & 1.205E-04 & 2.652E-01 & 3.159E-05 & 5.575E-02 & 5.037E-05 & 6.576E-02 & 9.507E-05 & 1.005E-01 & 4.219E-05 & 4.352E-02 & 2.424E-05 & 1.950E-02 & 4.004E-05 & 2.647E-02 & 8.686E-05 & 5.291E-02 & 1.063E-04 & 3.910E-02 & 1.166E-04 & 3.951E-02 \\
57011.414 & 0.22 & 1.66 & 1.163E-04 & 2.560E-01 & 3.784E-05 & 6.646E-02 & 4.951E-05 & 6.531E-02 & 9.895E-05 & 1.067E-01 & 4.031E-05 & 4.299E-02 & 2.006E-05 & 1.629E-02 & 3.841E-05 & 2.582E-02 & 9.103E-05 & 5.564E-02 & 1.007E-04 & 3.731E-02 & 1.081E-04 & 3.689E-02 \\
57011.430 & 0.20 & 1.77 & 1.105E-04 & 2.787E-01 & 3.300E-05 & 6.609E-02 & 4.430E-05 & 6.586E-02 & 8.483E-05 & 1.048E-01 & 3.869E-05 & 4.436E-02 & 2.162E-05 & 1.937E-02 & 3.689E-05 & 2.732E-02 & 7.572E-05 & 5.182E-02 & 9.465E-05 & 3.890E-02 & 1.023E-04 & 3.869E-02 \\
57011.441 & 0.18 & 1.84 & 1.061E-04 & 2.827E-01 & 3.448E-05 & 7.300E-02 & 4.069E-05 & 6.555E-02 & 7.452E-05 & 9.998E-02 & 3.711E-05 & 4.606E-02 & 2.268E-05 & 2.143E-02 & 3.423E-05 & 2.728E-02 & 7.592E-05 & 5.479E-02 & 8.671E-05 & 3.785E-02 & 9.600E-05 & 3.853E-02 \\
57012.375 & 0.19 & 1.80 & 1.083E-04 & 2.826E-01 & 3.555E-05 & 7.130E-02 & 4.516E-05 & 6.876E-02 & 8.376E-05 & 1.065E-01 & 3.944E-05 & 4.692E-02 & 1.938E-05 & 1.797E-02 & 3.742E-05 & 2.851E-02 & 7.565E-05 & 5.258E-02 & 8.931E-05 & 3.817E-02 & 1.011E-04 & 3.920E-02 \\
57012.387 & 0.19 & 1.80 & 1.085E-04 & 2.745E-01 & 3.847E-05 & 7.724E-02 & 4.466E-05 & 6.881E-02 & 8.301E-05 & 1.077E-01 & 3.524E-05 & 4.264E-02 & 2.246E-05 & 2.084E-02 & 3.414E-05 & 2.643E-02 & 7.939E-05 & 5.436E-02 & 9.163E-05 & 3.895E-02 & 9.798E-05 & 3.842E-02 \\
57012.402 & 0.17 & 1.93 & 8.437E-05 & 2.469E-01 & 3.455E-05 & 7.936E-02 & 4.050E-05 & 6.865E-02 & 8.316E-05 & 1.159E-01 & 3.219E-05 & 4.374E-02 & 2.043E-05 & 2.149E-02 & 2.835E-05 & 2.505E-02 & 6.629E-05 & 5.230E-02 & 7.872E-05 & 3.777E-02 & 8.723E-05 & 3.869E-02 \\
57012.414 & 0.17 & 1.93 & 9.822E-05 & 2.918E-01 & 3.061E-05 & 7.074E-02 & 3.791E-05 & 6.602E-02 & 7.904E-05 & 1.126E-01 & 3.170E-05 & 4.253E-02 & 1.615E-05 & 1.701E-02 & 2.746E-05 & 2.414E-02 & 6.620E-05 & 5.217E-02 & 7.519E-05 & 3.595E-02 & 8.359E-05 & 3.672E-02 \\
57013.414 & 0.07 & 2.96 & 4.443E-05 & 2.331E-01 & 1.434E-05 & 6.297E-02 & 1.864E-05 & 6.781E-02 & 3.120E-05 & 9.316E-02 & 9.570E-06 & 3.020E-02 & 4.600E-06 & 1.176E-02 & 1.121E-05 & 2.377E-02 & 1.613E-05 & 3.250E-02 & 2.216E-05 & 2.873E-02 & 2.316E-05 & 2.707E-02 \\
57013.426 & 0.06 & 2.98 & 3.459E-05 & 1.865E-01 & 1.265E-05 & 5.777E-02 & 1.683E-05 & 6.306E-02 & 3.602E-05 & 1.181E-01 & 9.820E-06 & 3.157E-02 & 5.660E-06 & 1.450E-02 & 1.234E-05 & 2.549E-02 & 1.401E-05 & 2.852E-02 & 2.503E-05 & 3.207E-02 & 2.586E-05 & 3.036E-02 \\
57013.438 & 0.07 & 2.96 & 1.510E-05 & 8.395E-02 & 2.341E-05 & 1.010E-01 & 1.626E-05 & 6.059E-02 & 2.968E-05 & 9.900E-02 & 1.114E-05 & 3.055E-02 & 6.700E-06 & 1.704E-02 & 1.127E-05 & 2.410E-02 & 1.253E-05 & 2.511E-02 & 2.624E-05 & 3.326E-02 & 2.728E-05 & 3.192E-02 \\
57013.449 & 0.07 & 2.93 & 2.092E-05 & 1.122E-01 & 1.255E-05 & 5.542E-02 & 1.842E-05 & 6.606E-02 & 3.132E-05 & 9.470E-02 & 1.104E-05 & 2.854E-02 & 5.070E-06 & 1.260E-02 & 1.163E-05 & 2.332E-02 & 1.552E-05 & 2.987E-02 & 2.399E-05 & 2.981E-02 & 2.736E-05 & 3.046E-02 \\
57020.391 & 0.11 & 2.44 & 8.901E-05 & 3.453E-01 & 2.455E-05 & 8.018E-02 & 3.271E-05 & 8.066E-02 & 5.850E-05 & 1.254E-01 & 2.172E-05 & 4.448E-02 & 1.141E-05 & 1.837E-02 & 2.084E-05 & 2.756E-02 & 4.358E-05 & 5.364E-02 & 4.930E-05 & 3.743E-02 & 5.975E-05 & 4.141E-02 \\
57020.402 & 0.11 & 2.40 & 9.069E-05 & 3.483E-01 & 3.196E-05 & 9.763E-02 & 3.411E-05 & 8.160E-02 & 6.353E-05 & 1.323E-01 & 2.273E-05 & 4.598E-02 & 1.200E-05 & 1.910E-02 & 2.172E-05 & 2.828E-02 & 4.304E-05 & 5.264E-02 & 5.000E-05 & 3.735E-02 & 6.348E-05 & 4.274E-02 \\
57020.414 & 0.10 & 2.45 & 6.718E-05 & 2.800E-01 & 2.290E-05 & 7.786E-02 & 3.122E-05 & 7.998E-02 & 5.966E-05 & 1.263E-01 & 2.327E-05 & 4.854E-02 & 1.235E-05 & 2.095E-02 & 2.243E-05 & 3.067E-02 & 4.022E-05 & 5.208E-02 & 4.830E-05 & 3.837E-02 & 5.635E-05 & 4.068E-02 \\
57020.426 & 0.10 & 2.46 & 7.301E-05 & 3.063E-01 & 2.032E-05 & 6.867E-02 & 2.990E-05 & 7.674E-02 & 5.195E-05 & 1.093E-01 & 1.920E-05 & 4.199E-02 & 1.258E-05 & 2.131E-02 & 2.136E-05 & 2.926E-02 & 4.519E-05 & 5.660E-02 & 5.165E-05 & 3.991E-02 & 5.456E-05 & 3.910E-02 \\
57021.332 & 0.09 & 2.62 & 6.118E-05 & 2.882E-01 & 1.948E-05 & 7.495E-02 & 2.712E-05 & 7.808E-02 & 4.311E-05 & 1.086E-01 & 1.781E-05 & 4.343E-02 & 1.129E-05 & 2.177E-02 & 1.875E-05 & 2.932E-02 & 3.112E-05 & 4.649E-02 & 4.127E-05 & 3.724E-02 & 4.962E-05 & 4.011E-02 \\
57021.344 & 0.08 & 2.69 & 6.309E-05 & 3.134E-01 & 2.455E-05 & 9.591E-02 & 2.465E-05 & 7.853E-02 & 4.571E-05 & 1.201E-01 & 1.511E-05 & 4.160E-02 & 7.590E-06 & 1.579E-02 & 1.683E-05 & 2.846E-02 & 3.093E-05 & 4.836E-02 & 3.827E-05 & 3.633E-02 & 4.580E-05 & 3.965E-02 \\
57021.355 & 0.09 & 2.64 & 6.464E-05 & 3.005E-01 & 2.513E-05 & 9.525E-02 & 2.636E-05 & 8.021E-02 & 4.828E-05 & 1.189E-01 & 1.712E-05 & 4.093E-02 & 9.420E-06 & 1.883E-02 & 2.001E-05 & 3.223E-02 & 3.245E-05 & 4.892E-02 & 4.179E-05 & 3.843E-02 & 4.565E-05 & 3.853E-02 \\
57021.371 & 0.09 & 2.61 & 7.167E-05 & 3.192E-01 & 3.128E-05 & 1.121E-01 & 2.722E-05 & 7.870E-02 & 5.098E-05 & 1.269E-01 & 1.912E-05 & 4.495E-02 & 1.063E-05 & 2.026E-02 & 1.793E-05 & 2.823E-02 & 3.078E-05 & 4.574E-02 & 4.032E-05 & 3.645E-02 & 4.572E-05 & 3.765E-02 \\
57029.379 & 0.21 & 1.70 & 1.627E-04 & 3.750E-01 & 5.371E-05 & 9.559E-02 & 6.356E-05 & 8.514E-02 & 1.210E-04 & 1.358E-01 & 4.936E-05 & 5.466E-02 & 2.519E-05 & 2.105E-02 & 4.604E-05 & 3.179E-02 & 9.571E-05 & 6.031E-02 & 1.099E-04 & 4.304E-02 & 1.234E-04 & 4.390E-02 \\
57029.391 & 0.21 & 1.70 & 1.748E-04 & 3.988E-01 & 4.258E-05 & 7.712E-02 & 6.461E-05 & 8.640E-02 & 1.165E-04 & 1.328E-01 & 5.148E-05 & 5.585E-02 & 2.527E-05 & 2.103E-02 & 4.275E-05 & 2.958E-02 & 9.442E-05 & 6.021E-02 & 1.197E-04 & 4.631E-02 & 1.239E-04 & 4.387E-02 \\
57029.402 & 0.20 & 1.73 & 1.738E-04 & 3.972E-01 & 4.370E-05 & 7.992E-02 & 6.088E-05 & 8.401E-02 & 1.218E-04 & 1.395E-01 & 4.661E-05 & 5.293E-02 & 2.759E-05 & 2.332E-02 & 4.252E-05 & 2.985E-02 & 9.281E-05 & 6.008E-02 & 1.140E-04 & 4.523E-02 & 1.232E-04 & 4.456E-02 \\
57029.414 & 0.20 & 1.75 & 1.639E-04 & 3.926E-01 & 5.699E-05 & 1.034E-01 & 5.863E-05 & 8.283E-02 & 1.128E-04 & 1.316E-01 & 4.476E-05 & 5.269E-02 & 2.348E-05 & 2.050E-02 & 4.066E-05 & 2.938E-02 & 9.045E-05 & 6.058E-02 & 1.061E-04 & 4.362E-02 & 1.147E-04 & 4.273E-02 \\
57030.336 & 0.17 & 1.95 & 1.289E-04 & 3.615E-01 & 3.779E-05 & 8.429E-02 & 4.662E-05 & 7.922E-02 & 8.542E-05 & 1.251E-01 & 3.740E-05 & 5.127E-02 & 1.752E-05 & 1.872E-02 & 3.298E-05 & 2.900E-02 & 7.074E-05 & 5.518E-02 & 8.217E-05 & 4.010E-02 & 9.145E-05 & 4.033E-02 \\
57030.348 & 0.16 & 2.02 & 1.090E-04 & 3.412E-01 & 3.968E-05 & 9.368E-02 & 4.137E-05 & 7.767E-02 & 7.125E-05 & 1.126E-01 & 3.052E-05 & 4.803E-02 & 1.695E-05 & 1.947E-02 & 2.799E-05 & 2.668E-02 & 6.313E-05 & 5.466E-02 & 8.365E-05 & 4.265E-02 & 8.242E-05 & 3.913E-02 \\
57030.363 & 0.16 & 2.00 & 1.019E-04 & 3.181E-01 & 3.998E-05 & 9.498E-02 & 4.476E-05 & 8.084E-02 & 8.363E-05 & 1.224E-01 & 3.348E-05 & 5.031E-02 & 1.733E-05 & 1.957E-02 & 3.278E-05 & 3.000E-02 & 6.436E-05 & 5.444E-02 & 7.779E-05 & 4.009E-02 & 8.340E-05 & 3.887E-02 \\
57030.375 & 0.15 & 2.04 & 1.064E-04 & 3.338E-01 & 2.797E-05 & 7.167E-02 & 4.339E-05 & 8.307E-02 & 7.774E-05 & 1.256E-01 & 3.034E-05 & 4.755E-02 & 1.669E-05 & 1.920E-02 & 2.819E-05 & 2.715E-02 & 6.206E-05 & 5.339E-02 & 8.243E-05 & 4.288E-02 & 8.728E-05 & 4.132E-02 \\
57031.332 & 0.21 & 1.68 & 1.464E-04 & 3.493E-01 & 4.533E-05 & 8.467E-02 & 5.510E-05 & 7.682E-02 & 1.055E-04 & 1.224E-01 & 4.448E-05 & 4.910E-02 & 2.621E-05 & 2.155E-02 & 3.294E-05 & 2.292E-02 & 8.657E-05 & 5.481E-02 & 1.060E-04 & 4.056E-02 & 1.183E-04 & 4.114E-02 \\
57031.344 & 0.21 & 1.72 & 1.420E-04 & 3.512E-01 & 4.078E-05 & 8.021E-02 & 5.309E-05 & 7.642E-02 & 9.905E-05 & 1.169E-01 & 4.034E-05 & 4.743E-02 & 2.045E-05 & 1.798E-02 & 3.798E-05 & 2.743E-02 & 8.484E-05 & 5.559E-02 & 1.012E-04 & 4.023E-02 & 1.122E-04 & 4.032E-02 \\
57031.359 & 0.22 & 1.64 & 1.360E-04 & 3.161E-01 & 4.706E-05 & 8.285E-02 & 5.245E-05 & 6.946E-02 & 1.054E-04 & 1.152E-01 & 4.300E-05 & 4.734E-02 & 2.359E-05 & 1.883E-02 & 4.305E-05 & 2.857E-02 & 8.955E-05 & 5.416E-02 & 1.088E-04 & 4.005E-02 & 1.214E-04 & 4.074E-02 \\
57031.371 & 0.22 & 1.67 & 1.389E-04 & 3.223E-01 & 5.920E-05 & 1.040E-01 & 5.701E-05 & 7.701E-02 & 9.995E-05 & 1.146E-01 & 4.336E-05 & 4.772E-02 & 2.393E-05 & 1.910E-02 & 3.736E-05 & 2.571E-02 & 8.775E-05 & 5.388E-02 & 1.043E-04 & 3.892E-02 & 1.155E-04 & 3.927E-02 \\
57032.332 & 0.13 & 2.19 & 8.102E-05 & 2.513E-01 & 3.623E-05 & 9.040E-02 & 3.366E-05 & 6.735E-02 & 6.384E-05 & 1.096E-01 & 2.562E-05 & 4.097E-02 & 1.365E-05 & 1.754E-02 & 2.313E-05 & 2.503E-02 & 4.034E-05 & 4.019E-02 & 5.916E-05 & 3.654E-02 & 5.543E-05 & 3.178E-02 \\
57032.348 & 0.15 & 2.03 & 1.138E-04 & 2.941E-01 & 3.322E-05 & 7.193E-02 & 3.910E-05 & 6.606E-02 & 7.829E-05 & 1.115E-01 & 3.008E-05 & 4.169E-02 & 1.457E-05 & 1.601E-02 & 2.717E-05 & 2.416E-02 & 5.046E-05 & 4.322E-02 & 6.547E-05 & 3.478E-02 & 7.147E-05 & 3.495E-02 \\
57032.359 & 0.15 & 2.05 & 9.868E-05 & 2.629E-01 & 3.385E-05 & 7.443E-02 & 3.624E-05 & 6.178E-02 & 7.125E-05 & 1.063E-01 & 2.732E-05 & 4.015E-02 & 1.346E-05 & 1.527E-02 & 2.748E-05 & 2.578E-02 & 4.931E-05 & 4.310E-02 & 6.429E-05 & 3.482E-02 & 7.399E-05 & 3.681E-02 \\
57032.371 & 0.15 & 2.03 & 8.793E-05 & 2.387E-01 & 2.875E-05 & 6.492E-02 & 3.722E-05 & 6.530E-02 & 7.867E-05 & 1.143E-01 & 2.884E-05 & 4.218E-02 & 1.517E-05 & 1.711E-02 & 2.636E-05 & 2.487E-02 & 5.115E-05 & 4.426E-02 & 6.434E-05 & 3.503E-02 & 7.227E-05 & 3.587E-02 \\
57033.383 & 0.28 & 1.38 & 1.770E-04 & 2.885E-01 & 6.305E-05 & 8.057E-02 & 7.038E-05 & 6.888E-02 & 1.422E-04 & 1.160E-01 & 5.763E-05 & 4.454E-02 & 3.061E-05 & 1.860E-02 & 4.661E-05 & 2.392E-02 & 9.666E-05 & 4.460E-02 & 1.267E-04 & 3.707E-02 & 1.367E-04 & 3.693E-02 \\
57033.398 & 0.26 & 1.44 & 1.657E-04 & 2.991E-01 & 6.769E-05 & 8.932E-02 & 6.891E-05 & 7.187E-02 & 1.335E-04 & 1.168E-01 & 5.141E-05 & 4.395E-02 & 3.177E-05 & 2.060E-02 & 5.101E-05 & 2.754E-02 & 9.529E-05 & 4.687E-02 & 1.229E-04 & 3.749E-02 & 1.324E-04 & 3.725E-02 \\
57033.418 & 0.25 & 1.49 & 1.796E-04 & 3.318E-01 & 5.288E-05 & 7.772E-02 & 6.509E-05 & 7.221E-02 & 1.255E-04 & 1.172E-01 & 5.381E-05 & 4.766E-02 & 3.009E-05 & 2.081E-02 & 4.773E-05 & 2.702E-02 & 8.894E-05 & 4.666E-02 & 1.241E-04 & 3.990E-02 & 1.308E-04 & 3.855E-02 \\
57033.438 & 0.25 & 1.49 & 1.839E-04 & 3.372E-01 & 5.078E-05 & 7.527E-02 & 6.775E-05 & 7.427E-02 & 1.242E-04 & 1.136E-01 & 5.231E-05 & 4.650E-02 & 3.210E-05 & 2.173E-02 & 5.044E-05 & 2.818E-02 & 9.438E-05 & 4.852E-02 & 1.299E-04 & 4.100E-02 & 1.388E-04 & 4.065E-02 \\
57034.309 & 0.25 & 1.48 & 1.522E-04 & 2.652E-01 & 5.100E-05 & 6.913E-02 & 6.383E-05 & 6.683E-02 & 1.206E-04 & 1.060E-01 & 4.827E-05 & 4.192E-02 & 2.918E-05 & 1.941E-02 & 4.003E-05 & 2.245E-02 & 8.698E-05 & 4.388E-02 & 1.159E-04 & 3.749E-02 & 1.322E-04 & 3.921E-02 \\
57034.324 & 0.25 & 1.49 & 1.578E-04 & 2.735E-01 & 4.681E-05 & 6.446E-02 & 6.779E-05 & 7.102E-02 & 1.203E-04 & 1.080E-01 & 4.920E-05 & 4.245E-02 & 2.617E-05 & 1.746E-02 & 4.602E-05 & 2.557E-02 & 8.430E-05 & 4.368E-02 & 1.174E-04 & 3.829E-02 & 1.278E-04 & 3.829E-02 \\
57034.344 & 0.26 & 1.48 & 1.590E-04 & 2.757E-01 & 6.100E-05 & 8.194E-02 & 6.633E-05 & 6.816E-02 & 1.302E-04 & 1.146E-01 & 5.128E-05 & 4.410E-02 & 2.753E-05 & 1.820E-02 & 4.870E-05 & 2.662E-02 & 8.160E-05 & 4.195E-02 & 1.166E-04 & 3.760E-02 & 1.282E-04 & 3.806E-02 \\
57034.363 & 0.26 & 1.45 & 1.817E-04 & 2.949E-01 & 5.381E-05 & 7.089E-02 & 7.131E-05 & 7.092E-02 & 1.331E-04 & 1.115E-01 & 5.075E-05 & 4.260E-02 & 3.001E-05 & 1.926E-02 & 5.038E-05 & 2.682E-02 & 8.724E-05 & 4.370E-02 & 1.154E-04 & 3.635E-02 & 1.316E-04 & 3.812E-02 \\
57035.230 & 0.21 & 1.70 & 1.655E-04 & 3.826E-01 & 4.220E-05 & 7.713E-02 & 5.961E-05 & 7.885E-02 & 1.192E-04 & 1.326E-01 & 4.624E-05 & 5.083E-02 & 2.642E-05 & 2.131E-02 & 4.329E-05 & 2.938E-02 & 9.534E-05 & 5.828E-02 & 1.107E-04 & 4.263E-02 & 1.254E-04 & 4.443E-02 \\
57035.242 & 0.23 & 1.61 & 1.784E-04 & 3.756E-01 & 5.168E-05 & 8.461E-02 & 6.692E-05 & 8.131E-02 & 1.267E-04 & 1.307E-01 & 5.046E-05 & 5.083E-02 & 2.899E-05 & 2.200E-02 & 4.740E-05 & 2.985E-02 & 1.013E-04 & 5.743E-02 & 1.216E-04 & 4.341E-02 & 1.332E-04 & 4.364E-02 \\
57035.254 & 0.23 & 1.59 & 1.998E-04 & 3.991E-01 & 5.571E-05 & 8.808E-02 & 7.023E-05 & 8.253E-02 & 1.231E-04 & 1.230E-01 & 5.208E-05 & 5.104E-02 & 2.934E-05 & 2.166E-02 & 4.637E-05 & 2.876E-02 & 1.027E-04 & 5.713E-02 & 1.239E-04 & 4.317E-02 & 1.375E-04 & 4.381E-02 \\
57035.266 & 0.24 & 1.57 & 1.845E-04 & 3.736E-01 & 5.157E-05 & 8.073E-02 & 6.974E-05 & 8.122E-02 & 1.382E-04 & 1.340E-01 & 5.314E-05 & 5.077E-02 & 3.167E-05 & 2.295E-02 & 4.862E-05 & 2.944E-02 & 1.041E-04 & 5.678E-02 & 1.329E-04 & 4.573E-02 & 1.381E-04 & 4.318E-02 \\
57036.426 & 0.19 & 1.79 & 1.422E-04 & 3.885E-01 & 3.833E-05 & 8.146E-02 & 5.325E-05 & 8.270E-02 & 1.008E-04 & 1.278E-01 & 3.988E-05 & 4.693E-02 & 2.227E-05 & 2.087E-02 & 3.784E-05 & 2.908E-02 & 8.379E-05 & 5.876E-02 & 1.058E-04 & 4.422E-02 & 1.181E-04 & 4.480E-02 \\
57036.438 & 0.18 & 1.87 & 1.340E-04 & 3.913E-01 & 3.368E-05 & 7.824E-02 & 5.185E-05 & 8.700E-02 & 8.866E-05 & 1.255E-01 & 4.153E-05 & 5.432E-02 & 2.205E-05 & 2.188E-02 & 3.460E-05 & 2.884E-02 & 8.067E-05 & 5.942E-02 & 9.574E-05 & 4.275E-02 & 1.018E-04 & 4.159E-02 \\
57036.449 & 0.20 & 1.77 & 1.544E-04 & 3.994E-01 & 4.210E-05 & 8.636E-02 & 5.628E-05 & 8.453E-02 & 1.139E-04 & 1.393E-01 & 4.461E-05 & 5.391E-02 & 2.612E-05 & 2.361E-02 & 3.869E-05 & 2.881E-02 & 8.555E-05 & 5.825E-02 & 1.074E-04 & 4.373E-02 & 1.203E-04 & 4.427E-02 \\
57036.461 & 0.20 & 1.77 & 1.415E-04 & 3.737E-01 & 4.182E-05 & 8.606E-02 & 5.712E-05 & 8.472E-02 & 9.744E-05 & 1.236E-01 & 4.421E-05 & 5.315E-02 & 2.368E-05 & 2.151E-02 & 4.099E-05 & 3.003E-02 & 8.355E-05 & 5.666E-02 & 1.128E-04 & 4.563E-02 & 1.201E-04 & 4.448E-02 \\
57037.191 & 0.23 & 1.59 & 1.935E-04 & 3.244E-01 & 5.209E-05 & 8.099E-02 & 5.665E-05 & 6.695E-02 & 1.100E-04 & 1.028E-01 & 3.884E-05 & 3.321E-02 & 2.832E-05 & 1.928E-02 & 5.010E-05 & 2.903E-02 & 8.856E-05 & 4.731E-02 & 1.103E-04 & 3.967E-02 & 1.212E-04 & 4.037E-02 \\
57037.203 & 0.20 & 1.75 & 1.529E-04 & 3.897E-01 & 4.246E-05 & 8.446E-02 & 5.588E-05 & 8.168E-02 & 9.832E-05 & 1.193E-01 & 4.348E-05 & 5.184E-02 & 2.002E-05 & 1.788E-02 & 4.302E-05 & 3.132E-02 & 8.882E-05 & 5.841E-02 & 1.077E-04 & 4.311E-02 & 1.157E-04 & 4.272E-02 \\
57037.215 & 0.20 & 1.77 & 1.519E-04 & 3.978E-01 & 4.043E-05 & 8.181E-02 & 5.614E-05 & 8.374E-02 & 9.793E-05 & 1.221E-01 & 4.283E-05 & 5.170E-02 & 2.154E-05 & 1.958E-02 & 3.917E-05 & 2.935E-02 & 9.252E-05 & 6.123E-02 & 1.088E-04 & 4.457E-02 & 1.185E-04 & 4.444E-02 \\
57037.227 & 0.20 & 1.75 & 1.464E-04 & 3.841E-01 & 4.588E-05 & 8.964E-02 & 5.539E-05 & 8.129E-02 & 1.011E-04 & 1.252E-01 & 4.492E-05 & 5.224E-02 & 2.762E-05 & 2.458E-02 & 4.155E-05 & 3.051E-02 & 9.506E-05 & 6.248E-02 & 1.031E-04 & 4.162E-02 & 1.214E-04 & 4.481E-02 \\
\enddata
\end{deluxetable*}
\end{longrotatetable}

